Parallelization of the inverse fast multipole method with an application to boundary element method

We present an algorithm to parallelize the inverse fast multipole method (IFMM), which is an approximate direct solver for dense linear systems. The parallel scheme is based on a greedy coloring algorithm, where two nodes in the hierarchy with the same color are separated by at least $\sigma$ nodes. We proved that when $\sigma \ge 6$, the workload associated with one color is embarrassingly parallel. However, the number of nodes in a group (color) may be small when $\sigma = 6$. Therefore, we also explored $\sigma = 3$, where a small fraction of the algorithm needs to be serialized, and the overall parallel efficiency was improved. We implemented the parallel IFMM using OpenMP for shared-memory machines. Successively, we applied it to a fast-multipole accelerated boundary element method (FMBEM) as a preconditioner, and compared its efficiency with (a) the original IFMM parallelized by linking a multi-threaded linear algebra library and (b) the commonly used parallel block-diagonal preconditioner. Our results showed that our parallel IFMM achieved at most $4\times$ and $11\times$ speedups over the reference method (a) and (b), respectively, in realistic examples involving more than one million variables.

==> 181031/office/office05--ngauss4-jpre-tol1e-5-maxepc040-delta7-inc0.tex <==
%% PWD: /home/ttaka/Dropbox/papers/helm3d/parallel/paper/181031/office
%% DATE: Wed Nov 28 11:24:02 JST 2018
%% root_ref: /home/ttaka/study/helm3d/181031/bigmem
%% exe_ref: fmm3logBDX4
%% jpre_ref: 3
%% tail_ref: ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0
\begin{tabular}{M}
\myheader\myheaderFlag
\renewcommand{\arraystretch}{\myarraystretch}


==> 181031/office/office05-fmm3logXsep3top2sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{262.34}\\
3 & \prtime{174.003}\\
4 & \prtime{60.836}\\
5 & \prtime{39.9453}\\
6 & \prtime{29.4859}\\
7 & \prtime{83.0809}\\
\midrule
 & \prtime{ 655.771486}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 655.771486} & \prtime{262.34} & \prtime{174.003} & \prtime{60.836} & \prtime{39.9453} & \prtime{29.4859} & \prtime{83.0809}&\prtime{ 974.397379}\\


==> 181031/office/office05-fmm3logXsep3top2sub0-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{374.587}\\
3 & \prtime{299.736}\\
4 & \prtime{113.689}\\
5 & \prtime{71.3283}\\
6 & \prtime{50.9255}\\
7 & \prtime{131.0599}\\
\midrule
 & \prtime{ 1047.367778}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub0-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 1047.367778} & \prtime{374.587} & \prtime{299.736} & \prtime{113.689} & \prtime{71.3283} & \prtime{50.9255} & \prtime{131.0599}&\prtime{ 1504.570095}\\


==> 181031/office/office05-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{59.3751}\\
3 & \prtime{42.038}\\
4 & \prtime{25.6614}\\
5 & \prtime{23.4065}\\
6 & \prtime{36.8812}\\
7 & \prtime{51.5531}\\
\midrule
 & \prtime{ 244.869556}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 244.869556} & \prtime{59.3751} & \prtime{42.038} & \prtime{25.6614} & \prtime{23.4065} & \prtime{36.8812} & \prtime{51.5531}&\prtime{ 912.671435}\\


==> 181031/office/office05-fmm3logXsep3top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{127.167}\\
3 & \prtime{69.096}\\
4 & \prtime{40.6989}\\
5 & \prtime{26.4218}\\
6 & \prtime{43.0548}\\
7 & \prtime{57.2434}\\
\midrule
 & \prtime{ 369.742576}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 369.742576} & \prtime{127.167} & \prtime{69.096} & \prtime{40.6989} & \prtime{26.4218} & \prtime{43.0548} & \prtime{57.2434}&\prtime{ 905.642425}\\


==> 181031/office/office05-fmm3logXsep3top2sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{243.532}\\
3 & \prtime{152.914}\\
4 & \prtime{61.7948}\\
5 & \prtime{39.9961}\\
6 & \prtime{67.3839}\\
\midrule
 & \prtime{ 567.116269}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 567.116269} & \prtime{243.532} & \prtime{152.914} & \prtime{61.7948} & \prtime{39.9961} & \prtime{67.3839}& &\prtime{ 198.228492}\\


==> 181031/office/office05-fmm3logXsep3top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{375.389}\\
3 & \prtime{299.482}\\
4 & \prtime{114.841}\\
5 & \prtime{68.1004}\\
6 & \prtime{107.5491}\\
\midrule
 & \prtime{ 966.858624}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 966.858624} & \prtime{375.389} & \prtime{299.482} & \prtime{114.841} & \prtime{68.1004} & \prtime{107.5491}& &\prtime{ 318.450868}\\


==> 181031/office/office05-fmm3logXsep3top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{62.1308}\\
3 & \prtime{41.0103}\\
4 & \prtime{25.0651}\\
5 & \prtime{23.4026}\\
6 & \prtime{49.5009}\\
\midrule
 & \prtime{ 202.594210}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 202.594210} & \prtime{62.1308} & \prtime{41.0103} & \prtime{25.0651} & \prtime{23.4026} & \prtime{49.5009}& &\prtime{ 148.054623}\\


==> 181031/office/office05-fmm3logXsep3top2sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1036.86}\\
3 & \prtime{640.886}\\
4 & \prtime{311.175}\\
5 & \prtime{164.377}\\
6 & \prtime{340.473}\\
\midrule
 & \prtime{ 2495.347091}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 2495.347091} & \prtime{1036.86} & \prtime{640.886} & \prtime{311.175} & \prtime{164.377} & \prtime{340.473}& &\prtime{ 818.407940}\\


==> 181031/office/office05-fmm3logXsep3top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{118.606}\\
3 & \prtime{65.8314}\\
4 & \prtime{39.755}\\
5 & \prtime{28.5375}\\
6 & \prtime{67.9361}\\
\midrule
 & \prtime{ 322.154945}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 322.154945} & \prtime{118.606} & \prtime{65.8314} & \prtime{39.755} & \prtime{28.5375} & \prtime{67.9361}& &\prtime{ 156.602083}\\


==> 181031/office/office05-fmm3logXsep3top2sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{224.913}\\
3 & \prtime{129.206}\\
4 & \prtime{69.6482}\\
5 & \prtime{227.5702}\\
\midrule
 & \prtime{ 651.703964}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 651.703964} & \prtime{224.913} & \prtime{129.206} & \prtime{69.6482} & \prtime{227.5702}& & &\prtime{ 213.955195}\\


==> 181031/office/office05-fmm3logXsep3top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{372.142}\\
3 & \prtime{298.277}\\
4 & \prtime{112.799}\\
5 & \prtime{161.9777}\\
\midrule
 & \prtime{ 945.586238}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 945.586238} & \prtime{372.142} & \prtime{298.277} & \prtime{112.799} & \prtime{161.9777}& & &\prtime{ 267.017424}\\


==> 181031/office/office05-fmm3logXsep3top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{58.1809}\\
3 & \prtime{41.1806}\\
4 & \prtime{33.725}\\
5 & \prtime{157.4234}\\
\midrule
 & \prtime{ 290.880123}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 290.880123} & \prtime{58.1809} & \prtime{41.1806} & \prtime{33.725} & \prtime{157.4234}& & &\prtime{ 192.535514}\\


==> 181031/office/office05-fmm3logXsep3top2sub2-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{911.581}\\
3 & \prtime{612.501}\\
4 & \prtime{305.222}\\
5 & \prtime{327.944}\\
\midrule
 & \prtime{ 2157.646191}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub2-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 2157.646191} & \prtime{911.581} & \prtime{612.501} & \prtime{305.222} & \prtime{327.944}& & &\prtime{ 500.382233}\\


==> 181031/office/office05-fmm3logXsep3top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{118.97}\\
3 & \prtime{62.9475}\\
4 & \prtime{47.6506}\\
5 & \prtime{174.2278}\\
\midrule
 & \prtime{ 404.170062}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 404.170062} & \prtime{118.97} & \prtime{62.9475} & \prtime{47.6506} & \prtime{174.2278}& & &\prtime{ 199.055015}\\


==> 181031/office/office05-fmm3logXsep3top2sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{234.476}\\
3 & \prtime{191.125}\\
4 & \prtime{1950.8539}\\
\midrule
 & \prtime{ 2376.545644}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 2376.545644} & \prtime{234.476} & \prtime{191.125} & \prtime{1950.8539}& & & &\prtime{ 1333.879931}\\


==> 181031/office/office05-fmm3logXsep3top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{481.748}\\
3 & \prtime{331.419}\\
4 & \prtime{1690.4176}\\
\midrule
 & \prtime{ 2503.889830}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 2503.889830} & \prtime{481.748} & \prtime{331.419} & \prtime{1690.4176}& & & &\prtime{ 1407.484725}\\


==> 181031/office/office05-fmm3logXsep3top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{58.5174}\\
3 & \prtime{68.4751}\\
4 & \prtime{1864.1245}\\
\midrule
 & \prtime{ 1991.205883}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 1991.205883} & \prtime{58.5174} & \prtime{68.4751} & \prtime{1864.1245}& & & &\prtime{ 1283.651962}\\


==> 181031/office/office05-fmm3logXsep3top2sub3-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{929.95}\\
3 & \prtime{672.491}\\
4 & \prtime{1901.526}\\
\midrule
 & \prtime{ 3504.085163}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub3-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 3504.085163} & \prtime{929.95} & \prtime{672.491} & \prtime{1901.526}& & & &\prtime{ 1641.957896}\\


==> 181031/office/office05-fmm3logXsep3top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{111.743}\\
3 & \prtime{102.842}\\
4 & \prtime{1886.0994}\\
\midrule
 & \prtime{ 2100.772626}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 2100.772626} & \prtime{111.743} & \prtime{102.842} & \prtime{1886.0994}& & & &\prtime{ 1296.579271}\\


==> 181031/office/office05-fmm3logXsep3top3sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{85.5796}\\
3 & \prtime{173.644}\\
4 & \prtime{60.8316}\\
5 & \prtime{39.7849}\\
6 & \prtime{28.3873}\\
7 & \prtime{84.7615}\\
\midrule
 & \prtime{ 478.953342}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 478.953342} & \prtime{85.5796} & \prtime{173.644} & \prtime{60.8316} & \prtime{39.7849} & \prtime{28.3873} & \prtime{84.7615}&\prtime{ 926.489067}\\


==> 181031/office/office05-fmm3logXsep3top3sub0-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{102.468}\\
3 & \prtime{300.53}\\
4 & \prtime{114.371}\\
5 & \prtime{74.5359}\\
6 & \prtime{48.9949}\\
7 & \prtime{144.8735}\\
\midrule
 & \prtime{ 791.918081}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub0-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 791.918081} & \prtime{102.468} & \prtime{300.53} & \prtime{114.371} & \prtime{74.5359} & \prtime{48.9949} & \prtime{144.8735}&\prtime{ 1559.699233}\\


==> 181031/office/office05-fmm3logXsep3top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{16.144}\\
3 & \prtime{41.9346}\\
4 & \prtime{25.3954}\\
5 & \prtime{23.3985}\\
6 & \prtime{37.2497}\\
7 & \prtime{50.8505}\\
\midrule
 & \prtime{ 200.989983}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 200.989983} & \prtime{16.144} & \prtime{41.9346} & \prtime{25.3954} & \prtime{23.3985} & \prtime{37.2497} & \prtime{50.8505}&\prtime{ 923.194430}\\


==> 181031/office/office05-fmm3logXsep3top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{36.5668}\\
3 & \prtime{69.0308}\\
4 & \prtime{40.9546}\\
5 & \prtime{26.712}\\
6 & \prtime{40.8032}\\
7 & \prtime{55.3626}\\
\midrule
 & \prtime{ 275.436193}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 275.436193} & \prtime{36.5668} & \prtime{69.0308} & \prtime{40.9546} & \prtime{26.712} & \prtime{40.8032} & \prtime{55.3626}&\prtime{ 919.106143}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.80893}\\
3 & \prtime{5.72098}\\
4 & \prtime{4.45867}\\
5 & \prtime{7.76158}\\
6 & \prtime{34.3052}\\
\midrule
 & \prtime{ 55.496151}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 55.496151} & \prtime{1.80893} & \prtime{5.72098} & \prtime{4.45867} & \prtime{7.76158} & \prtime{34.3052}& &\prtime{ 214.921886}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{17.1093}\\
3 & \prtime{49.2664}\\
4 & \prtime{25.9987}\\
5 & \prtime{21.9984}\\
6 & \prtime{47.0702}\\
\midrule
 & \prtime{ 162.946386}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 162.946386} & \prtime{17.1093} & \prtime{49.2664} & \prtime{25.9987} & \prtime{21.9984} & \prtime{47.0702}& &\prtime{ 204.874075}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{56.4335}\\
3 & \prtime{153.829}\\
4 & \prtime{62.1743}\\
5 & \prtime{38.862}\\
6 & \prtime{60.3461}\\
\midrule
 & \prtime{ 373.140776}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 373.140776} & \prtime{56.4335} & \prtime{153.829} & \prtime{62.1743} & \prtime{38.862} & \prtime{60.3461}& &\prtime{ 189.904565}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.47097}\\
3 & \prtime{9.44619}\\
4 & \prtime{9.75251}\\
5 & \prtime{16.5733}\\
6 & \prtime{72.6244}\\
\midrule
 & \prtime{ 112.356120}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 112.356120} & \prtime{2.47097} & \prtime{9.44619} & \prtime{9.75251} & \prtime{16.5733} & \prtime{72.6244}& &\prtime{ 293.328488}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{15.7619}\\
3 & \prtime{86.2595}\\
4 & \prtime{42.5913}\\
5 & \prtime{39.0919}\\
6 & \prtime{92.8646}\\
\midrule
 & \prtime{ 278.006596}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 278.006596} & \prtime{15.7619} & \prtime{86.2595} & \prtime{42.5913} & \prtime{39.0919} & \prtime{92.8646}& &\prtime{ 330.540053}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{79.3665}\\
3 & \prtime{301.543}\\
4 & \prtime{114.014}\\
5 & \prtime{66.7481}\\
6 & \prtime{117.3099}\\
\midrule
 & \prtime{ 680.497701}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 680.497701} & \prtime{79.3665} & \prtime{301.543} & \prtime{114.014} & \prtime{66.7481} & \prtime{117.3099}& &\prtime{ 322.414508}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.6199}\\
3 & \prtime{4.10611}\\
4 & \prtime{2.87382}\\
5 & \prtime{4.68215}\\
6 & \prtime{21.4344}\\
\midrule
 & \prtime{ 36.162830}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 36.162830} & \prtime{1.6199} & \prtime{4.10611} & \prtime{2.87382} & \prtime{4.68215} & \prtime{21.4344}& &\prtime{ 141.923494}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{8.89475}\\
3 & \prtime{22.4982}\\
4 & \prtime{14.4985}\\
5 & \prtime{13.1683}\\
6 & \prtime{26.3339}\\
\midrule
 & \prtime{ 86.867856}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 86.867856} & \prtime{8.89475} & \prtime{22.4982} & \prtime{14.4985} & \prtime{13.1683} & \prtime{26.3339}& &\prtime{ 150.686307}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{17.4992}\\
3 & \prtime{41.101}\\
4 & \prtime{25.0404}\\
5 & \prtime{23.1472}\\
6 & \prtime{50.7327}\\
\midrule
 & \prtime{ 159.005325}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 159.005325} & \prtime{17.4992} & \prtime{41.101} & \prtime{25.0404} & \prtime{23.1472} & \prtime{50.7327}& &\prtime{ 144.312507}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{31.8825}\\
3 & \prtime{23.2856}\\
4 & \prtime{129.803}\\
5 & \prtime{69.979}\\
6 & \prtime{268.7377}\\
\midrule
 & \prtime{ 525.164595}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 525.164595} & \prtime{31.8825} & \prtime{23.2856} & \prtime{129.803} & \prtime{69.979} & \prtime{268.7377}& &\prtime{ 878.600819}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{110.41}\\
3 & \prtime{152.235}\\
4 & \prtime{136.046}\\
5 & \prtime{92.8203}\\
6 & \prtime{326.276}\\
\midrule
 & \prtime{ 819.346975}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 819.346975} & \prtime{110.41} & \prtime{152.235} & \prtime{136.046} & \prtime{92.8203} & \prtime{326.276}& &\prtime{ 862.041764}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{707.982}\\
3 & \prtime{642.125}\\
4 & \prtime{287.416}\\
5 & \prtime{168.962}\\
6 & \prtime{379.131}\\
\midrule
 & \prtime{ 2187.230380}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 2187.230380} & \prtime{707.982} & \prtime{642.125} & \prtime{287.416} & \prtime{168.962} & \prtime{379.131}& &\prtime{ 997.176338}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.69276}\\
3 & \prtime{5.91225}\\
4 & \prtime{3.49808}\\
5 & \prtime{5.25051}\\
6 & \prtime{25.8912}\\
\midrule
 & \prtime{ 43.737408}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 43.737408} & \prtime{1.69276} & \prtime{5.91225} & \prtime{3.49808} & \prtime{5.25051} & \prtime{25.8912}& &\prtime{ 152.362973}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{13.2334}\\
3 & \prtime{37.0174}\\
4 & \prtime{19.5462}\\
5 & \prtime{15.8903}\\
6 & \prtime{33.4922}\\
\midrule
 & \prtime{ 120.649218}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 120.649218} & \prtime{13.2334} & \prtime{37.0174} & \prtime{19.5462} & \prtime{15.8903} & \prtime{33.4922}& &\prtime{ 151.246384}\\


==> 181031/office/office05-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{24.6037}\\
3 & \prtime{65.7879}\\
4 & \prtime{40.2333}\\
5 & \prtime{28.6748}\\
6 & \prtime{70.1926}\\
\midrule
 & \prtime{ 231.002488}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 231.002488} & \prtime{24.6037} & \prtime{65.7879} & \prtime{40.2333} & \prtime{28.6748} & \prtime{70.1926}& &\prtime{ 143.667136}\\


==> 181031/office/office05-fmm3logXsep3top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{43.2542}\\
3 & \prtime{129.605}\\
4 & \prtime{69.4873}\\
5 & \prtime{229.513}\\
\midrule
 & \prtime{ 472.227730}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 472.227730} & \prtime{43.2542} & \prtime{129.605} & \prtime{69.4873} & \prtime{229.513}& & &\prtime{ 214.913130}\\


==> 181031/office/office05-fmm3logXsep3top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{70.3249}\\
3 & \prtime{297.461}\\
4 & \prtime{112.758}\\
5 & \prtime{151.0284}\\
\midrule
 & \prtime{ 631.951745}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 631.951745} & \prtime{70.3249} & \prtime{297.461} & \prtime{112.758} & \prtime{151.0284}& & &\prtime{ 263.788999}\\


==> 181031/office/office05-fmm3logXsep3top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{12.6429}\\
3 & \prtime{41.6529}\\
4 & \prtime{33.5507}\\
5 & \prtime{157.1495}\\
\midrule
 & \prtime{ 245.365224}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 245.365224} & \prtime{12.6429} & \prtime{41.6529} & \prtime{33.5507} & \prtime{157.1495}& & &\prtime{ 193.443850}\\


==> 181031/office/office05-fmm3logXsep3top3sub2-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{394.449}\\
3 & \prtime{613.106}\\
4 & \prtime{313.665}\\
5 & \prtime{342.299}\\
\midrule
 & \prtime{ 1663.919287}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub2-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 1663.919287} & \prtime{394.449} & \prtime{613.106} & \prtime{313.665} & \prtime{342.299}& & &\prtime{ 491.391456}\\


==> 181031/office/office05-fmm3logXsep3top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{36.7354}\\
3 & \prtime{62.9896}\\
4 & \prtime{48.4499}\\
5 & \prtime{178.9987}\\
\midrule
 & \prtime{ 327.547943}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 327.547943} & \prtime{36.7354} & \prtime{62.9896} & \prtime{48.4499} & \prtime{178.9987}& & &\prtime{ 201.757999}\\


==> 181031/office/office05-fmm3logXsep3top3sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{80.8234}\\
3 & \prtime{190.047}\\
4 & \prtime{1967.0036}\\
\midrule
 & \prtime{ 2237.955549}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 2237.955549} & \prtime{80.8234} & \prtime{190.047} & \prtime{1967.0036}& & & &\prtime{ 1325.982357}\\


==> 181031/office/office05-fmm3logXsep3top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{129.362}\\
3 & \prtime{325.107}\\
4 & \prtime{1684.6886}\\
\midrule
 & \prtime{ 2139.234148}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 2139.234148} & \prtime{129.362} & \prtime{325.107} & \prtime{1684.6886}& & & &\prtime{ 1406.018542}\\


==> 181031/office/office05-fmm3logXsep3top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{20.2815}\\
3 & \prtime{67.2968}\\
4 & \prtime{1832.1045}\\
\midrule
 & \prtime{ 1919.759638}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 1919.759638} & \prtime{20.2815} & \prtime{67.2968} & \prtime{1832.1045}& & & &\prtime{ 1277.566463}\\


==> 181031/office/office05-fmm3logXsep3top3sub3-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{598.789}\\
3 & \prtime{666.668}\\
4 & \prtime{1893.9613}\\
\midrule
 & \prtime{ 3159.529504}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub3-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 3159.529504} & \prtime{598.789} & \prtime{666.668} & \prtime{1893.9613}& & & &\prtime{ 1616.672640}\\


==> 181031/office/office05-fmm3logXsep3top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{39.3114}\\
3 & \prtime{101.606}\\
4 & \prtime{1887.7257}\\
\midrule
 & \prtime{ 2028.725056}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep3top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 2028.725056} & \prtime{39.3114} & \prtime{101.606} & \prtime{1887.7257}& & & &\prtime{ 1289.902536}\\


==> 181031/office/office05-fmm3logXsep6top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{71.1632}\\
3 & \prtime{431.742}\\
4 & \prtime{220.633}\\
5 & \prtime{76.4173}\\
6 & \prtime{57.1832}\\
\midrule
 & \prtime{ 858.610595}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b6 & \prtime{ 858.610595} & \prtime{71.1632} & \prtime{431.742} & \prtime{220.633} & \prtime{76.4173} & \prtime{57.1832}& &\prtime{ 204.286971}\\


==> 181031/office/office05-fmm3logXsep6top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{88.6141}\\
3 & \prtime{914.527}\\
4 & \prtime{399.319}\\
5 & \prtime{115.005}\\
6 & \prtime{107.2816}\\
\midrule
 & \prtime{ 1626.284388}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b6 & \prtime{ 1626.284388} & \prtime{88.6141} & \prtime{914.527} & \prtime{399.319} & \prtime{115.005} & \prtime{107.2816}& &\prtime{ 318.846824}\\


==> 181031/office/office05-fmm3logXsep6top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{13.1565}\\
3 & \prtime{138.563}\\
4 & \prtime{88.4578}\\
5 & \prtime{45.8044}\\
6 & \prtime{34.7654}\\
\midrule
 & \prtime{ 322.213890}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b6 & \prtime{ 322.213890} & \prtime{13.1565} & \prtime{138.563} & \prtime{88.4578} & \prtime{45.8044} & \prtime{34.7654}& &\prtime{ 149.546261}\\


==> 181031/office/office05-fmm3logXsep6top3sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{490.038}\\
3 & \prtime{1535.35}\\
4 & \prtime{744.94}\\
5 & \prtime{247.572}\\
6 & \prtime{388.160}\\
\midrule
 & \prtime{ 3407.574026}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b6 & \prtime{ 3407.574026} & \prtime{490.038} & \prtime{1535.35} & \prtime{744.94} & \prtime{247.572} & \prtime{388.160}& &\prtime{ 818.434722}\\


==> 181031/office/office05-fmm3logXsep6top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{27.1578}\\
3 & \prtime{221.396}\\
4 & \prtime{146.005}\\
5 & \prtime{52.4011}\\
6 & \prtime{46.8850}\\
\midrule
 & \prtime{ 495.330299}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b6 & \prtime{ 495.330299} & \prtime{27.1578} & \prtime{221.396} & \prtime{146.005} & \prtime{52.4011} & \prtime{46.8850}& &\prtime{ 147.483900}\\


==> 181031/office/office05-fmm3logXsep6top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{59.805}\\
3 & \prtime{388.109}\\
4 & \prtime{254.422}\\
5 & \prtime{229.3102}\\
\midrule
 & \prtime{ 932.023871}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b5 & \prtime{ 932.023871} & \prtime{59.805} & \prtime{388.109} & \prtime{254.422} & \prtime{229.3102}& & &\prtime{ 211.475709}\\


==> 181031/office/office05-fmm3logXsep6top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{89.0187}\\
3 & \prtime{911.783}\\
4 & \prtime{389.938}\\
5 & \prtime{228.350}\\
\midrule
 & \prtime{ 1619.458053}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b5 & \prtime{ 1619.458053} & \prtime{89.0187} & \prtime{911.783} & \prtime{389.938} & \prtime{228.350}& & &\prtime{ 260.510611}\\


==> 181031/office/office05-fmm3logXsep6top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{13.718}\\
3 & \prtime{133.862}\\
4 & \prtime{127.662}\\
5 & \prtime{177.9007}\\
\midrule
 & \prtime{ 453.516663}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b5 & \prtime{ 453.516663} & \prtime{13.718} & \prtime{133.862} & \prtime{127.662} & \prtime{177.9007}& & &\prtime{ 192.635871}\\


==> 181031/office/office05-fmm3logXsep6top3sub2-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{425.879}\\
3 & \prtime{1521.44}\\
4 & \prtime{789.19}\\
5 & \prtime{413.083}\\
\midrule
 & \prtime{ 3150.016357}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub2-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b5 & \prtime{ 3150.016357} & \prtime{425.879} & \prtime{1521.44} & \prtime{789.19} & \prtime{413.083}& & &\prtime{ 489.793970}\\


==> 181031/office/office05-fmm3logXsep6top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{21.8226}\\
3 & \prtime{210.994}\\
4 & \prtime{179.913}\\
5 & \prtime{196.5626}\\
\midrule
 & \prtime{ 609.687843}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsep6top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b5 & \prtime{ 609.687843} & \prtime{21.8226} & \prtime{210.994} & \prtime{179.913} & \prtime{196.5626}& & &\prtime{ 199.140982}\\


==> 181031/office/office05-fmm3logXsub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{95.1315}\\
3 & \prtime{116.32}\\
4 & \prtime{246.041}\\
5 & \prtime{600.616}\\
6 & \prtime{453.074}\\
7 & \prtime{165.9998}\\
\midrule
 & \prtime{ 1683.013525}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 1683.013525} & \prtime{95.1315} & \prtime{116.32} & \prtime{246.041} & \prtime{600.616} & \prtime{453.074} & \prtime{165.9998}&\prtime{ 915.901331}\\


==> 181031/office/office05-fmm3logXsub0-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{182.728}\\
3 & \prtime{320.676}\\
4 & \prtime{446.32}\\
5 & \prtime{891.629}\\
6 & \prtime{604.23}\\
7 & \prtime{218.7402}\\
\midrule
 & \prtime{ 2670.298439}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub0-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 2670.298439} & \prtime{182.728} & \prtime{320.676} & \prtime{446.32} & \prtime{891.629} & \prtime{604.23} & \prtime{218.7402}&\prtime{ 1129.238365}\\


==> 181031/office/office05-fmm3logXsub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{13.94}\\
3 & \prtime{52.3417}\\
4 & \prtime{142.154}\\
5 & \prtime{452.657}\\
6 & \prtime{398.956}\\
7 & \prtime{132.5589}\\
\midrule
 & \prtime{ 1198.494555}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 1198.494555} & \prtime{13.94} & \prtime{52.3417} & \prtime{142.154} & \prtime{452.657} & \prtime{398.956} & \prtime{132.5589}&\prtime{ 919.583050}\\


==> 181031/office/office05-fmm3logXsub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{43.2749}\\
3 & \prtime{67.4759}\\
4 & \prtime{193.193}\\
5 & \prtime{533.342}\\
6 & \prtime{410.495}\\
7 & \prtime{137.7399}\\
\midrule
 & \prtime{ 1391.642795}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 1391.642795} & \prtime{43.2749} & \prtime{67.4759} & \prtime{193.193} & \prtime{533.342} & \prtime{410.495} & \prtime{137.7399}&\prtime{ 897.361349}\\


==> 181031/office/office05-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.92488}\\
3 & \prtime{17.6813}\\
4 & \prtime{51.099}\\
5 & \prtime{151.921}\\
6 & \prtime{268.7002}\\
\midrule
 & \prtime{ 496.727835}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 496.727835} & \prtime{5.92488} & \prtime{17.6813} & \prtime{51.099} & \prtime{151.921} & \prtime{268.7002}& &\prtime{ 201.948180}\\


==> 181031/office/office05-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{87.8686}\\
3 & \prtime{117.729}\\
4 & \prtime{241.051}\\
5 & \prtime{564.244}\\
6 & \prtime{447.1152}\\
\midrule
 & \prtime{ 1459.410273}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 1459.410273} & \prtime{87.8686} & \prtime{117.729} & \prtime{241.051} & \prtime{564.244} & \prtime{447.1152}& &\prtime{ 208.536751}\\


==> 181031/office/office05-fmm3logXsub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{96.3538}\\
3 & \prtime{285.833}\\
4 & \prtime{394.022}\\
5 & \prtime{739.406}\\
6 & \prtime{608.6475}\\
\midrule
 & \prtime{ 2125.669857}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 2125.669857} & \prtime{96.3538} & \prtime{285.833} & \prtime{394.022} & \prtime{739.406} & \prtime{608.6475}& &\prtime{ 310.863524}\\


==> 181031/office/office05-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{3.26075}\\
3 & \prtime{13.7762}\\
4 & \prtime{45.5125}\\
5 & \prtime{117.902}\\
6 & \prtime{233.7875}\\
\midrule
 & \prtime{ 415.625421}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 415.625421} & \prtime{3.26075} & \prtime{13.7762} & \prtime{45.5125} & \prtime{117.902} & \prtime{233.7875}& &\prtime{ 136.518601}\\


==> 181031/office/office05-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{13.9069}\\
3 & \prtime{48.8016}\\
4 & \prtime{138.308}\\
5 & \prtime{446.421}\\
6 & \prtime{380.424}\\
\midrule
 & \prtime{ 1029.283336}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 1029.283336} & \prtime{13.9069} & \prtime{48.8016} & \prtime{138.308} & \prtime{446.421} & \prtime{380.424}& &\prtime{ 151.926306}\\


==> 181031/office/office05-fmm3logXsub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{13.7045}\\
3 & \prtime{56.1216}\\
4 & \prtime{300.711}\\
5 & \prtime{502.912}\\
6 & \prtime{899.737}\\
\midrule
 & \prtime{ 1774.598457}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 1774.598457} & \prtime{13.7045} & \prtime{56.1216} & \prtime{300.711} & \prtime{502.912} & \prtime{899.737}& &\prtime{ 830.035877}\\


==> 181031/office/office05-fmm3logXsub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{382.947}\\
3 & \prtime{1002.9}\\
4 & \prtime{1093.05}\\
5 & \prtime{3218.26}\\
6 & \prtime{1634.844}\\
\midrule
 & \prtime{ 7333.412046}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub1-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 7333.412046} & \prtime{382.947} & \prtime{1002.9} & \prtime{1093.05} & \prtime{3218.26} & \prtime{1634.844}& &\prtime{ 829.843476}\\


==> 181031/office/office05-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.82509}\\
3 & \prtime{16.5568}\\
4 & \prtime{48.3855}\\
5 & \prtime{122.205}\\
6 & \prtime{240.3029}\\
\midrule
 & \prtime{ 430.750310}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 430.750310} & \prtime{1.82509} & \prtime{16.5568} & \prtime{48.3855} & \prtime{122.205} & \prtime{240.3029}& &\prtime{ 154.266960}\\


==> 181031/office/office05-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{27.8029}\\
3 & \prtime{65.4329}\\
4 & \prtime{185.366}\\
5 & \prtime{507.454}\\
6 & \prtime{403.5902}\\
\midrule
 & \prtime{ 1191.041369}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 1191.041369} & \prtime{27.8029} & \prtime{65.4329} & \prtime{185.366} & \prtime{507.454} & \prtime{403.5902}& &\prtime{ 146.061951}\\


==> 181031/office/office05-fmm3logXsub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{191.574}\\
3 & \prtime{175.531}\\
4 & \prtime{258.891}\\
5 & \prtime{1191.4475}\\
\midrule
 & \prtime{ 1817.831412}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 1817.831412} & \prtime{191.574} & \prtime{175.531} & \prtime{258.891} & \prtime{1191.4475}& & &\prtime{ 213.204019}\\


==> 181031/office/office05-fmm3logXsub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{90.3271}\\
3 & \prtime{279.212}\\
4 & \prtime{359.445}\\
5 & \prtime{966.2418}\\
\midrule
 & \prtime{ 1695.586640}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 1695.586640} & \prtime{90.3271} & \prtime{279.212} & \prtime{359.445} & \prtime{966.2418}& & &\prtime{ 261.316701}\\


==> 181031/office/office05-fmm3logXsub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{13.1334}\\
3 & \prtime{53.9184}\\
4 & \prtime{161.398}\\
5 & \prtime{982.9971}\\
\midrule
 & \prtime{ 1211.834628}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 1211.834628} & \prtime{13.1334} & \prtime{53.9184} & \prtime{161.398} & \prtime{982.9971}& & &\prtime{ 194.837080}\\


==> 181031/office/office05-fmm3logXsub2-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{274.257}\\
3 & \prtime{628.845}\\
4 & \prtime{1053.01}\\
5 & \prtime{1646.045}\\
\midrule
 & \prtime{ 3602.519315}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub2-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 3602.519315} & \prtime{274.257} & \prtime{628.845} & \prtime{1053.01} & \prtime{1646.045}& & &\prtime{ 508.022671}\\


==> 181031/office/office05-fmm3logXsub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{32.3504}\\
3 & \prtime{79.4127}\\
4 & \prtime{207.598}\\
5 & \prtime{1083.6501}\\
\midrule
 & \prtime{ 1403.400548}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 1403.400548} & \prtime{32.3504} & \prtime{79.4127} & \prtime{207.598} & \prtime{1083.6501}& & &\prtime{ 200.301664}\\


==> 181031/office/office05-fmm3logXsub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{63.235}\\
3 & \prtime{220.522}\\
4 & \prtime{6170.3358}\\
\midrule
 & \prtime{ 6454.196107}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 6454.196107} & \prtime{63.235} & \prtime{220.522} & \prtime{6170.3358}& & & &\prtime{ 1328.725033}\\


==> 181031/office/office05-fmm3logXsub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{87.7927}\\
3 & \prtime{495.969}\\
4 & \prtime{5006.6997}\\
\midrule
 & \prtime{ 5590.570312}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 5590.570312} & \prtime{87.7927} & \prtime{495.969} & \prtime{5006.6997}& & & &\prtime{ 1408.335013}\\


==> 181031/office/office05-fmm3logXsub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{17.9122}\\
3 & \prtime{69.627}\\
4 & \prtime{5193.865}\\
\midrule
 & \prtime{ 5281.525157}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 5281.525157} & \prtime{17.9122} & \prtime{69.627} & \prtime{5193.865}& & & &\prtime{ 1282.071204}\\


==> 181031/office/office05-fmm3logXsub3-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{299.399}\\
3 & \prtime{637.032}\\
4 & \prtime{6527.8049}\\
\midrule
 & \prtime{ 7464.369197}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub3-dk64.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 7464.369197} & \prtime{299.399} & \prtime{637.032} & \prtime{6527.8049}& & & &\prtime{ 1654.859992}\\


==> 181031/office/office05-fmm3logXsub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{47.4997}\\
3 & \prtime{106.215}\\
4 & \prtime{5647.8645}\\
\midrule
 & \prtime{ 5801.692668}\\
\end{tabular}


==> 181031/office/office05-fmm3logXsub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 5801.692668} & \prtime{47.4997} & \prtime{106.215} & \prtime{5647.8645}& & & &\prtime{ 1296.399636}\\


==> 181031/sphereii/sphereii10--ngauss4-jpre-tol1e-5-maxepc040-delta7-inc95.tex <==
%% PWD: /home/ttaka/Dropbox/papers/helm3d/parallel/paper/181031/sphereii
%% DATE: Wed Nov 28 11:26:58 JST 2018
%% root_ref: /home/ttaka/study/helm3d/181031/g
%% exe_ref: fmm3logBDX2
%% jpre_ref: 3
%% tail_ref: ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95
\begin{tabular}{M}
\myheader\myheaderFlag
\renewcommand{\arraystretch}{\myarraystretch}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.0963923}\\
3 & \prtime{0.568583}\\
4 & \prtime{1.60519}\\
5 & \prtime{4.00718}\\
6 & \prtime{9.13979}\\
7 & \prtime{38.3887}\\
\midrule
 & \prtime{ 55.222969}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 55.222969} & \prtime{0.0963923} & \prtime{0.568583} & \prtime{1.60519} & \prtime{4.00718} & \prtime{9.13979} & \prtime{38.3887}&\prtime{ 100.452714}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.00637}\\
3 & \prtime{2.15961}\\
4 & \prtime{4.16409}\\
5 & \prtime{9.18002}\\
6 & \prtime{16.5149}\\
7 & \prtime{46.7181}\\
\midrule
 & \prtime{ 81.228458}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 81.228458} & \prtime{1.00637} & \prtime{2.15961} & \prtime{4.16409} & \prtime{9.18002} & \prtime{16.5149} & \prtime{46.7181}&\prtime{ 102.395777}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.64113}\\
3 & \prtime{5.62803}\\
4 & \prtime{8.51921}\\
5 & \prtime{16.8236}\\
6 & \prtime{39.9745}\\
7 & \prtime{46.8716}\\
\midrule
 & \prtime{ 124.886904}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.110219}\\
3 & \prtime{0.251996}\\
4 & \prtime{0.680971}\\
5 & \prtime{2.25866}\\
6 & \prtime{6.46186}\\
7 & \prtime{28.6636}\\
\midrule
 & \prtime{ 39.835221}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 39.835221} & \prtime{0.110219} & \prtime{0.251996} & \prtime{0.680971} & \prtime{2.25866} & \prtime{6.46186} & \prtime{28.6636}&\prtime{ 94.611164}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.573331}\\
3 & \prtime{0.86194}\\
4 & \prtime{1.94211}\\
5 & \prtime{5.29768}\\
6 & \prtime{12.2312}\\
7 & \prtime{33.3373}\\
\midrule
 & \prtime{ 55.652996}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 55.652996} & \prtime{0.573331} & \prtime{0.86194} & \prtime{1.94211} & \prtime{5.29768} & \prtime{12.2312} & \prtime{33.3373}&\prtime{ 97.987529}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{3.06478}\\
3 & \prtime{1.8747}\\
4 & \prtime{3.40909}\\
5 & \prtime{9.79881}\\
6 & \prtime{32.7931}\\
7 & \prtime{35.5828}\\
\midrule
 & \prtime{ 87.946381}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 87.946381} & \prtime{3.06478} & \prtime{1.8747} & \prtime{3.40909} & \prtime{9.79881} & \prtime{32.7931} & \prtime{35.5828}&\prtime{ 97.422032}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.124377}\\
3 & \prtime{0.458512}\\
4 & \prtime{0.93937}\\
5 & \prtime{2.59149}\\
6 & \prtime{7.24175}\\
7 & \prtime{30.6744}\\
\midrule
 & \prtime{ 43.453531}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 43.453531} & \prtime{0.124377} & \prtime{0.458512} & \prtime{0.93937} & \prtime{2.59149} & \prtime{7.24175} & \prtime{30.6744}&\prtime{ 95.930863}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.785895}\\
3 & \prtime{1.36132}\\
4 & \prtime{2.67336}\\
5 & \prtime{5.81501}\\
6 & \prtime{13.1456}\\
7 & \prtime{35.5748}\\
\midrule
 & \prtime{ 60.779663}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 60.779663} & \prtime{0.785895} & \prtime{1.36132} & \prtime{2.67336} & \prtime{5.81501} & \prtime{13.1456} & \prtime{35.5748}&\prtime{ 96.852532}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.15832}\\
3 & \prtime{8.00316}\\
4 & \prtime{5.31293}\\
5 & \prtime{11.1997}\\
6 & \prtime{33.2544}\\
7 & \prtime{37.9711}\\
\midrule
 & \prtime{ 101.367356}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b7 & \prtime{ 101.367356} & \prtime{4.15832} & \prtime{8.00316} & \prtime{5.31293} & \prtime{11.1997} & \prtime{33.2544} & \prtime{37.9711}&\prtime{ 99.391757}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.0867542}\\
3 & \prtime{0.562931}\\
4 & \prtime{1.64486}\\
5 & \prtime{4.1075}\\
6 & \prtime{23.01597}\\
\midrule
 & \prtime{ 29.788027}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 29.788027} & \prtime{0.0867542} & \prtime{0.562931} & \prtime{1.64486} & \prtime{4.1075} & \prtime{23.01597}& &\prtime{ 99.621359}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.16109}\\
3 & \prtime{2.09878}\\
4 & \prtime{4.31743}\\
5 & \prtime{8.71032}\\
6 & \prtime{25.7235}\\
\midrule
 & \prtime{ 42.383240}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 42.383240} & \prtime{1.16109} & \prtime{2.09878} & \prtime{4.31743} & \prtime{8.71032} & \prtime{25.7235}& &\prtime{ 101.133800}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.33013}\\
3 & \prtime{6.17701}\\
4 & \prtime{7.95789}\\
5 & \prtime{16.1394}\\
6 & \prtime{45.6436}\\
\midrule
 & \prtime{ 81.648971}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.101228}\\
3 & \prtime{1.61444}\\
4 & \prtime{4.48788}\\
5 & \prtime{9.02275}\\
6 & \prtime{38.4934}\\
\midrule
 & \prtime{ 54.090114}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 54.090114} & \prtime{0.101228} & \prtime{1.61444} & \prtime{4.48788} & \prtime{9.02275} & \prtime{38.4934}& &\prtime{ 122.326085}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.46877}\\
3 & \prtime{5.13908}\\
4 & \prtime{8.86163}\\
5 & \prtime{16.2266}\\
6 & \prtime{45.5489}\\
\midrule
 & \prtime{ 77.614947}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 77.614947} & \prtime{1.46877} & \prtime{5.13908} & \prtime{8.86163} & \prtime{16.2266} & \prtime{45.5489}& &\prtime{ 122.894184}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{8.79795}\\
3 & \prtime{13.7419}\\
4 & \prtime{18.2448}\\
5 & \prtime{27.6708}\\
6 & \prtime{50.7515}\\
\midrule
 & \prtime{ 119.588373}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 119.588373} & \prtime{8.79795} & \prtime{13.7419} & \prtime{18.2448} & \prtime{27.6708} & \prtime{50.7515}& &\prtime{ 124.530080}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.0966287}\\
3 & \prtime{0.233772}\\
4 & \prtime{0.649971}\\
5 & \prtime{2.19527}\\
6 & \prtime{15.45797}\\
\midrule
 & \prtime{ 19.005169}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 19.005169} & \prtime{0.0966287} & \prtime{0.233772} & \prtime{0.649971} & \prtime{2.19527} & \prtime{15.45797}& &\prtime{ 93.595973}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.544285}\\
3 & \prtime{0.80182}\\
4 & \prtime{1.89934}\\
5 & \prtime{5.3391}\\
6 & \prtime{18.19203}\\
\midrule
 & \prtime{ 27.147317}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 27.147317} & \prtime{0.544285} & \prtime{0.80182} & \prtime{1.89934} & \prtime{5.3391} & \prtime{18.19203}& &\prtime{ 91.883664}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.44467}\\
3 & \prtime{2.02331}\\
4 & \prtime{3.27811}\\
5 & \prtime{9.65715}\\
6 & \prtime{35.63923}\\
\midrule
 & \prtime{ 52.417465}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 52.417465} & \prtime{1.44467} & \prtime{2.02331} & \prtime{3.27811} & \prtime{9.65715} & \prtime{35.63923}& &\prtime{ 92.827500}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.107693}\\
3 & \prtime{0.431638}\\
4 & \prtime{0.904034}\\
5 & \prtime{2.60861}\\
6 & \prtime{16.98716}\\
\midrule
 & \prtime{ 21.422651}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 21.422651} & \prtime{0.107693} & \prtime{0.431638} & \prtime{0.904034} & \prtime{2.60861} & \prtime{16.98716}& &\prtime{ 92.644900}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.753818}\\
3 & \prtime{1.14644}\\
4 & \prtime{2.57256}\\
5 & \prtime{5.94471}\\
6 & \prtime{20.33126}\\
\midrule
 & \prtime{ 31.120189}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 31.120189} & \prtime{0.753818} & \prtime{1.14644} & \prtime{2.57256} & \prtime{5.94471} & \prtime{20.33126}& &\prtime{ 92.656509}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.3713}\\
3 & \prtime{2.60879}\\
4 & \prtime{5.03198}\\
5 & \prtime{10.8441}\\
6 & \prtime{37.23744}\\
\midrule
 & \prtime{ 58.482749}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b6 & \prtime{ 58.482749} & \prtime{2.3713} & \prtime{2.60879} & \prtime{5.03198} & \prtime{10.8441} & \prtime{37.23744}& &\prtime{ 93.541865}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.09969}\\
3 & \prtime{0.587986}\\
4 & \prtime{1.62611}\\
5 & \prtime{59.89495}\\
\midrule
 & \prtime{ 62.301866}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 62.301866} & \prtime{0.09969} & \prtime{0.587986} & \prtime{1.62611} & \prtime{59.89495}& & &\prtime{ 409.237009}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.983892}\\
3 & \prtime{2.02194}\\
4 & \prtime{4.00391}\\
5 & \prtime{63.33377}\\
\midrule
 & \prtime{ 70.437556}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 70.437556} & \prtime{0.983892} & \prtime{2.02194} & \prtime{4.00391} & \prtime{63.33377}& & &\prtime{ 408.029946}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.0602}\\
3 & \prtime{5.65707}\\
4 & \prtime{9.42954}\\
5 & \prtime{102.99858}\\
\midrule
 & \prtime{ 122.251087}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.0976723}\\
3 & \prtime{1.971}\\
4 & \prtime{4.87493}\\
5 & \prtime{72.5398}\\
\midrule
 & \prtime{ 79.579042}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 79.579042} & \prtime{0.0976723} & \prtime{1.971} & \prtime{4.87493} & \prtime{72.5398}& & &\prtime{ 433.848686}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.3034}\\
3 & \prtime{4.93998}\\
4 & \prtime{9.06251}\\
5 & \prtime{77.5374}\\
\midrule
 & \prtime{ 92.937066}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 92.937066} & \prtime{1.3034} & \prtime{4.93998} & \prtime{9.06251} & \prtime{77.5374}& & &\prtime{ 433.014174}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{10.2928}\\
3 & \prtime{15.8048}\\
4 & \prtime{17.3847}\\
5 & \prtime{88.8550}\\
\midrule
 & \prtime{ 132.431495}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 132.431495} & \prtime{10.2928} & \prtime{15.8048} & \prtime{17.3847} & \prtime{88.8550}& & &\prtime{ 457.968931}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.0955425}\\
3 & \prtime{0.235451}\\
4 & \prtime{0.651871}\\
5 & \prtime{53.99704}\\
\midrule
 & \prtime{ 55.073434}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 55.073434} & \prtime{0.0955425} & \prtime{0.235451} & \prtime{0.651871} & \prtime{53.99704}& & &\prtime{ 386.054178}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.538464}\\
3 & \prtime{0.779479}\\
4 & \prtime{1.86537}\\
5 & \prtime{56.13626}\\
\midrule
 & \prtime{ 59.414188}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 59.414188} & \prtime{0.538464} & \prtime{0.779479} & \prtime{1.86537} & \prtime{56.13626}& & &\prtime{ 386.697519}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.3045}\\
3 & \prtime{1.65189}\\
4 & \prtime{4.41862}\\
5 & \prtime{91.60678}\\
\midrule
 & \prtime{ 99.076959}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 99.076959} & \prtime{1.3045} & \prtime{1.65189} & \prtime{4.41862} & \prtime{91.60678}& & &\prtime{ 403.983147}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.112817}\\
3 & \prtime{0.380582}\\
4 & \prtime{0.893186}\\
5 & \prtime{55.00931}\\
\midrule
 & \prtime{ 56.490508}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 56.490508} & \prtime{0.112817} & \prtime{0.380582} & \prtime{0.893186} & \prtime{55.00931}& & &\prtime{ 408.103630}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.748423}\\
3 & \prtime{1.31108}\\
4 & \prtime{2.53141}\\
5 & \prtime{58.21852}\\
\midrule
 & \prtime{ 62.903778}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 62.903778} & \prtime{0.748423} & \prtime{1.31108} & \prtime{2.53141} & \prtime{58.21852}& & &\prtime{ 400.542505}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{3.89743}\\
3 & \prtime{2.41672}\\
4 & \prtime{6.36002}\\
5 & \prtime{97.43986}\\
\midrule
 & \prtime{ 110.211738}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b5 & \prtime{ 110.211738} & \prtime{3.89743} & \prtime{2.41672} & \prtime{6.36002} & \prtime{97.43986}& & &\prtime{ 426.293211}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.0880101}\\
3 & \prtime{0.589708}\\
4 & \prtime{621.2194}\\
\midrule
 & \prtime{ 621.920506}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 621.920506} & \prtime{0.0880101} & \prtime{0.589708} & \prtime{621.2194}& & & &\prtime{ 1731.042349}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.06572}\\
3 & \prtime{1.9248}\\
4 & \prtime{643.5544}\\
\midrule
 & \prtime{ 646.568465}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 646.568465} & \prtime{1.06572} & \prtime{1.9248} & \prtime{643.5544}& & & &\prtime{ 1706.112424}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.24479}\\
3 & \prtime{6.2789}\\
4 & \prtime{974.0007}\\
\midrule
 & \prtime{ 984.549876}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.0959912}\\
3 & \prtime{1.96787}\\
4 & \prtime{621.6825}\\
\midrule
 & \prtime{ 623.768950}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 623.768950} & \prtime{0.0959912} & \prtime{1.96787} & \prtime{621.6825}& & & &\prtime{ 1766.486121}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.19139}\\
3 & \prtime{4.47494}\\
4 & \prtime{645.3763}\\
\midrule
 & \prtime{ 651.066220}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 651.066220} & \prtime{1.19139} & \prtime{4.47494} & \prtime{645.3763}& & & &\prtime{ 1754.741281}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{10.824}\\
3 & \prtime{11.2036}\\
4 & \prtime{666.9218}\\
\midrule
 & \prtime{ 688.972387}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 688.972387} & \prtime{10.824} & \prtime{11.2036} & \prtime{666.9218}& & & &\prtime{ 1885.724816}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.0964293}\\
3 & \prtime{0.237069}\\
4 & \prtime{625.5387}\\
\midrule
 & \prtime{ 625.894781}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 625.894781} & \prtime{0.0964293} & \prtime{0.237069} & \prtime{625.5387}& & & &\prtime{ 1699.526181}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.566268}\\
3 & \prtime{1.26061}\\
4 & \prtime{632.3825}\\
\midrule
 & \prtime{ 634.233085}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 634.233085} & \prtime{0.566268} & \prtime{1.26061} & \prtime{632.3825}& & & &\prtime{ 1658.043192}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.16695}\\
3 & \prtime{2.43189}\\
4 & \prtime{929.5051}\\
\midrule
 & \prtime{ 933.127276}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 933.127276} & \prtime{1.16695} & \prtime{2.43189} & \prtime{929.5051}& & & &\prtime{ 1798.408147}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.108296}\\
3 & \prtime{0.402827}\\
4 & \prtime{615.509}\\
\midrule
 & \prtime{ 616.042863}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 616.042863} & \prtime{0.108296} & \prtime{0.402827} & \prtime{615.509}& & & &\prtime{ 1708.217481}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.755711}\\
3 & \prtime{1.57898}\\
4 & \prtime{627.9446}\\
\midrule
 & \prtime{ 630.301968}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 630.301968} & \prtime{0.755711} & \prtime{1.57898} & \prtime{627.9446}& & & &\prtime{ 1684.712477}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.96816}\\
3 & \prtime{3.90847}\\
4 & \prtime{946.8217}\\
\midrule
 & \prtime{ 952.721803}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t2b4 & \prtime{ 952.721803} & \prtime{1.96816} & \prtime{3.90847} & \prtime{946.8217}& & & &\prtime{ 1797.344662}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.273589}\\
3 & \prtime{0.593528}\\
4 & \prtime{1.64701}\\
5 & \prtime{4.0324}\\
6 & \prtime{9.3487}\\
7 & \prtime{39.0670}\\
\midrule
 & \prtime{ 56.394225}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 56.394225} & \prtime{0.273589} & \prtime{0.593528} & \prtime{1.64701} & \prtime{4.0324} & \prtime{9.3487} & \prtime{39.0670}&\prtime{ 99.774812}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.25453}\\
3 & \prtime{2.11154}\\
4 & \prtime{4.10512}\\
5 & \prtime{8.8389}\\
6 & \prtime{15.8406}\\
7 & \prtime{43.8649}\\
\midrule
 & \prtime{ 77.450598}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 77.450598} & \prtime{1.25453} & \prtime{2.11154} & \prtime{4.10512} & \prtime{8.8389} & \prtime{15.8406} & \prtime{43.8649}&\prtime{ 100.144037}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{7.48356}\\
3 & \prtime{5.70098}\\
4 & \prtime{8.64864}\\
5 & \prtime{17.0025}\\
6 & \prtime{39.9656}\\
7 & \prtime{48.2873}\\
\midrule
 & \prtime{ 128.582756}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.281675}\\
3 & \prtime{0.251766}\\
4 & \prtime{0.682572}\\
5 & \prtime{2.248}\\
6 & \prtime{6.51728}\\
7 & \prtime{28.8051}\\
\midrule
 & \prtime{ 40.201644}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 40.201644} & \prtime{0.281675} & \prtime{0.251766} & \prtime{0.682572} & \prtime{2.248} & \prtime{6.51728} & \prtime{28.8051}&\prtime{ 94.193965}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.936769}\\
3 & \prtime{0.839283}\\
4 & \prtime{1.95643}\\
5 & \prtime{5.25868}\\
6 & \prtime{12.1676}\\
7 & \prtime{33.7946}\\
\midrule
 & \prtime{ 56.383955}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 56.383955} & \prtime{0.936769} & \prtime{0.839283} & \prtime{1.95643} & \prtime{5.25868} & \prtime{12.1676} & \prtime{33.7946}&\prtime{ 97.147565}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{6.15212}\\
3 & \prtime{1.86304}\\
4 & \prtime{3.41809}\\
5 & \prtime{9.81316}\\
6 & \prtime{33.249}\\
7 & \prtime{36.1523}\\
\midrule
 & \prtime{ 92.084452}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 92.084452} & \prtime{6.15212} & \prtime{1.86304} & \prtime{3.41809} & \prtime{9.81316} & \prtime{33.249} & \prtime{36.1523}&\prtime{ 97.862076}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.270367}\\
3 & \prtime{0.407207}\\
4 & \prtime{0.91596}\\
5 & \prtime{2.59647}\\
6 & \prtime{7.18608}\\
7 & \prtime{30.3123}\\
\midrule
 & \prtime{ 43.095703}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 43.095703} & \prtime{0.270367} & \prtime{0.407207} & \prtime{0.91596} & \prtime{2.59647} & \prtime{7.18608} & \prtime{30.3123}&\prtime{ 95.656501}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.12386}\\
3 & \prtime{1.32431}\\
4 & \prtime{2.67021}\\
5 & \prtime{5.82523}\\
6 & \prtime{13.1168}\\
7 & \prtime{35.4248}\\
\midrule
 & \prtime{ 60.908977}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 60.908977} & \prtime{1.12386} & \prtime{1.32431} & \prtime{2.67021} & \prtime{5.82523} & \prtime{13.1168} & \prtime{35.4248}&\prtime{ 96.880817}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{3.31088}\\
3 & \prtime{8.05331}\\
4 & \prtime{5.37794}\\
5 & \prtime{11.2578}\\
6 & \prtime{33.9938}\\
7 & \prtime{38.2215}\\
\midrule
 & \prtime{ 101.741706}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b7 & \prtime{ 101.741706} & \prtime{3.31088} & \prtime{8.05331} & \prtime{5.37794} & \prtime{11.2578} & \prtime{33.9938} & \prtime{38.2215}&\prtime{ 98.983371}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.263512}\\
3 & \prtime{0.541166}\\
4 & \prtime{1.56355}\\
5 & \prtime{3.89801}\\
6 & \prtime{21.66546}\\
\midrule
 & \prtime{ 28.303396}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 28.303396} & \prtime{0.263512} & \prtime{0.541166} & \prtime{1.56355} & \prtime{3.89801} & \prtime{21.66546}& &\prtime{ 100.339969}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.50915}\\
3 & \prtime{2.09628}\\
4 & \prtime{4.30688}\\
5 & \prtime{9.11463}\\
6 & \prtime{25.5934}\\
\midrule
 & \prtime{ 43.004919}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 43.004919} & \prtime{1.50915} & \prtime{2.09628} & \prtime{4.30688} & \prtime{9.11463} & \prtime{25.5934}& &\prtime{ 101.159438}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.36098}\\
3 & \prtime{6.12108}\\
4 & \prtime{7.91494}\\
5 & \prtime{16.3276}\\
6 & \prtime{45.1346}\\
\midrule
 & \prtime{ 81.245963}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.257609}\\
3 & \prtime{1.96275}\\
4 & \prtime{4.76119}\\
5 & \prtime{8.80692}\\
6 & \prtime{38.2674}\\
\midrule
 & \prtime{ 54.427761}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 54.427761} & \prtime{0.257609} & \prtime{1.96275} & \prtime{4.76119} & \prtime{8.80692} & \prtime{38.2674}& &\prtime{ 120.835230}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.71044}\\
3 & \prtime{5.14082}\\
4 & \prtime{8.87083}\\
5 & \prtime{16.3741}\\
6 & \prtime{45.0316}\\
\midrule
 & \prtime{ 77.499269}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 77.499269} & \prtime{1.71044} & \prtime{5.14082} & \prtime{8.87083} & \prtime{16.3741} & \prtime{45.0316}& &\prtime{ 123.210710}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{8.993}\\
3 & \prtime{13.7819}\\
4 & \prtime{17.896}\\
5 & \prtime{27.637}\\
6 & \prtime{51.5268}\\
\midrule
 & \prtime{ 120.204830}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 120.204830} & \prtime{8.993} & \prtime{13.7819} & \prtime{17.896} & \prtime{27.637} & \prtime{51.5268}& &\prtime{ 124.130102}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.274137}\\
3 & \prtime{0.233282}\\
4 & \prtime{0.654834}\\
5 & \prtime{2.19729}\\
6 & \prtime{15.48836}\\
\midrule
 & \prtime{ 19.219539}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 19.219539} & \prtime{0.274137} & \prtime{0.233282} & \prtime{0.654834} & \prtime{2.19729} & \prtime{15.48836}& &\prtime{ 91.473360}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.85034}\\
3 & \prtime{0.802359}\\
4 & \prtime{1.90094}\\
5 & \prtime{5.31575}\\
6 & \prtime{18.08053}\\
\midrule
 & \prtime{ 27.318901}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 27.318901} & \prtime{0.85034} & \prtime{0.802359} & \prtime{1.90094} & \prtime{5.31575} & \prtime{18.08053}& &\prtime{ 91.732063}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.56535}\\
3 & \prtime{2.02545}\\
4 & \prtime{3.27252}\\
5 & \prtime{9.66665}\\
6 & \prtime{35.68606}\\
\midrule
 & \prtime{ 52.591109}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 52.591109} & \prtime{1.56535} & \prtime{2.02545} & \prtime{3.27252} & \prtime{9.66665} & \prtime{35.68606}& &\prtime{ 92.537145}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.258336}\\
3 & \prtime{0.438969}\\
4 & \prtime{0.900733}\\
5 & \prtime{2.55557}\\
6 & \prtime{17.55889}\\
\midrule
 & \prtime{ 22.082654}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 22.082654} & \prtime{0.258336} & \prtime{0.438969} & \prtime{0.900733} & \prtime{2.55557} & \prtime{17.55889}& &\prtime{ 92.367625}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.08984}\\
3 & \prtime{1.13331}\\
4 & \prtime{2.56573}\\
5 & \prtime{5.8891}\\
6 & \prtime{19.99851}\\
\midrule
 & \prtime{ 31.047996}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 31.047996} & \prtime{1.08984} & \prtime{1.13331} & \prtime{2.56573} & \prtime{5.8891} & \prtime{19.99851}& &\prtime{ 93.484994}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.30278}\\
3 & \prtime{2.59698}\\
4 & \prtime{5.01203}\\
5 & \prtime{10.8119}\\
6 & \prtime{37.28881}\\
\midrule
 & \prtime{ 58.390453}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b6 & \prtime{ 58.390453} & \prtime{2.30278} & \prtime{2.59698} & \prtime{5.01203} & \prtime{10.8119} & \prtime{37.28881}& &\prtime{ 93.466232}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.267575}\\
3 & \prtime{0.594844}\\
4 & \prtime{1.62937}\\
5 & \prtime{59.56415}\\
\midrule
 & \prtime{ 62.149445}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 62.149445} & \prtime{0.267575} & \prtime{0.594844} & \prtime{1.62937} & \prtime{59.56415}& & &\prtime{ 416.807339}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.19687}\\
3 & \prtime{2.1051}\\
4 & \prtime{4.04474}\\
5 & \prtime{63.3876}\\
\midrule
 & \prtime{ 70.830775}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 70.830775} & \prtime{1.19687} & \prtime{2.1051} & \prtime{4.04474} & \prtime{63.3876}& & &\prtime{ 414.861659}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{3.41884}\\
3 & \prtime{5.6525}\\
4 & \prtime{9.44492}\\
5 & \prtime{103.03944}\\
\midrule
 & \prtime{ 121.653466}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.247429}\\
3 & \prtime{1.94717}\\
4 & \prtime{5.1755}\\
5 & \prtime{71.9633}\\
\midrule
 & \prtime{ 79.431385}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 79.431385} & \prtime{0.247429} & \prtime{1.94717} & \prtime{5.1755} & \prtime{71.9633}& & &\prtime{ 436.698022}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.45043}\\
3 & \prtime{5.15343}\\
4 & \prtime{9.05224}\\
5 & \prtime{77.9345}\\
\midrule
 & \prtime{ 93.686238}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 93.686238} & \prtime{1.45043} & \prtime{5.15343} & \prtime{9.05224} & \prtime{77.9345}& & &\prtime{ 436.118402}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{12.8944}\\
3 & \prtime{15.794}\\
4 & \prtime{17.3872}\\
5 & \prtime{89.7532}\\
\midrule
 & \prtime{ 135.952341}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 135.952341} & \prtime{12.8944} & \prtime{15.794} & \prtime{17.3872} & \prtime{89.7532}& & &\prtime{ 445.341762}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.242775}\\
3 & \prtime{0.234594}\\
4 & \prtime{0.645359}\\
5 & \prtime{53.64348}\\
\midrule
 & \prtime{ 54.869306}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 54.869306} & \prtime{0.242775} & \prtime{0.234594} & \prtime{0.645359} & \prtime{53.64348}& & &\prtime{ 386.392266}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.838848}\\
3 & \prtime{0.776928}\\
4 & \prtime{1.87021}\\
5 & \prtime{56.14733}\\
\midrule
 & \prtime{ 59.729042}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 59.729042} & \prtime{0.838848} & \prtime{0.776928} & \prtime{1.87021} & \prtime{56.14733}& & &\prtime{ 386.996492}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.29843}\\
3 & \prtime{1.64624}\\
4 & \prtime{4.41688}\\
5 & \prtime{92.07843}\\
\midrule
 & \prtime{ 99.536686}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 99.536686} & \prtime{1.29843} & \prtime{1.64624} & \prtime{4.41688} & \prtime{92.07843}& & &\prtime{ 388.513856}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.254483}\\
3 & \prtime{0.381151}\\
4 & \prtime{0.895186}\\
5 & \prtime{54.90348}\\
\midrule
 & \prtime{ 56.530095}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 56.530095} & \prtime{0.254483} & \prtime{0.381151} & \prtime{0.895186} & \prtime{54.90348}& & &\prtime{ 411.289022}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.0378}\\
3 & \prtime{1.33434}\\
4 & \prtime{2.5499}\\
5 & \prtime{58.18674}\\
\midrule
 & \prtime{ 63.205314}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 63.205314} & \prtime{1.0378} & \prtime{1.33434} & \prtime{2.5499} & \prtime{58.18674}& & &\prtime{ 408.269021}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{7.8188}\\
3 & \prtime{2.42224}\\
4 & \prtime{6.34544}\\
5 & \prtime{97.03849}\\
\midrule
 & \prtime{ 113.724145}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b5 & \prtime{ 113.724145} & \prtime{7.8188} & \prtime{2.42224} & \prtime{6.34544} & \prtime{97.03849}& & &\prtime{ 413.353628}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.223929}\\
3 & \prtime{0.604207}\\
4 & \prtime{618.4537}\\
\midrule
 & \prtime{ 619.305098}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 619.305098} & \prtime{0.223929} & \prtime{0.604207} & \prtime{618.4537}& & & &\prtime{ 1766.076250}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.29576}\\
3 & \prtime{1.90668}\\
4 & \prtime{631.5916}\\
\midrule
 & \prtime{ 634.816988}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 634.816988} & \prtime{1.29576} & \prtime{1.90668} & \prtime{631.5916}& & & &\prtime{ 1763.610901}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.63972}\\
3 & \prtime{6.24653}\\
4 & \prtime{968.0817}\\
\midrule
 & \prtime{ 978.992829}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.246031}\\
3 & \prtime{2.03675}\\
4 & \prtime{621.2769}\\
\midrule
 & \prtime{ 623.582690}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 623.582690} & \prtime{0.246031} & \prtime{2.03675} & \prtime{621.2769}& & & &\prtime{ 1810.811066}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.31633}\\
3 & \prtime{4.73954}\\
4 & \prtime{639.708}\\
\midrule
 & \prtime{ 645.787423}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 645.787423} & \prtime{1.31633} & \prtime{4.73954} & \prtime{639.708}& & & &\prtime{ 1807.891611}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{9.24104}\\
3 & \prtime{11.2166}\\
4 & \prtime{662.9142}\\
\midrule
 & \prtime{ 683.394716}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 683.394716} & \prtime{9.24104} & \prtime{11.2166} & \prtime{662.9142}& & & &\prtime{ 1837.612262}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.243532}\\
3 & \prtime{0.23686}\\
4 & \prtime{621.3008}\\
\midrule
 & \prtime{ 621.804093}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 621.804093} & \prtime{0.243532} & \prtime{0.23686} & \prtime{621.3008}& & & &\prtime{ 1727.069212}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.862665}\\
3 & \prtime{1.26877}\\
4 & \prtime{631.4057}\\
\midrule
 & \prtime{ 633.561014}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 633.561014} & \prtime{0.862665} & \prtime{1.26877} & \prtime{631.4057}& & & &\prtime{ 1701.377281}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.23667}\\
3 & \prtime{2.43148}\\
4 & \prtime{933.5268}\\
\midrule
 & \prtime{ 937.219159}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 937.219159} & \prtime{1.23667} & \prtime{2.43148} & \prtime{933.5268}& & & &\prtime{ 1797.178811}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.260114}\\
3 & \prtime{0.399276}\\
4 & \prtime{614.895}\\
\midrule
 & \prtime{ 615.577916}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 615.577916} & \prtime{0.260114} & \prtime{0.399276} & \prtime{614.895}& & & &\prtime{ 1774.417330}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.03653}\\
3 & \prtime{1.58443}\\
4 & \prtime{625.9888}\\
\midrule
 & \prtime{ 628.633818}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 628.633818} & \prtime{1.03653} & \prtime{1.58443} & \prtime{625.9888}& & & &\prtime{ 1729.254398}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.72308}\\
3 & \prtime{3.89779}\\
4 & \prtime{943.9403}\\
\midrule
 & \prtime{ 949.585177}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t3b4 & \prtime{ 949.585177} & \prtime{1.72308} & \prtime{3.89779} & \prtime{943.9403}& & & &\prtime{ 1767.086074}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.265825}\\
3 & \prtime{1.63393}\\
4 & \prtime{1.62555}\\
5 & \prtime{3.97454}\\
6 & \prtime{9.17833}\\
7 & \prtime{38.5413}\\
\midrule
 & \prtime{ 56.640286}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b7 & \prtime{ 56.640286} & \prtime{0.265825} & \prtime{1.63393} & \prtime{1.62555} & \prtime{3.97454} & \prtime{9.17833} & \prtime{38.5413}&\prtime{ 99.027410}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.44588}\\
3 & \prtime{5.65396}\\
4 & \prtime{4.10044}\\
5 & \prtime{8.73544}\\
6 & \prtime{15.765}\\
7 & \prtime{43.9662}\\
\midrule
 & \prtime{ 81.105304}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b7 & \prtime{ 81.105304} & \prtime{1.44588} & \prtime{5.65396} & \prtime{4.10044} & \prtime{8.73544} & \prtime{15.765} & \prtime{43.9662}&\prtime{ 100.752635}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.89141}\\
3 & \prtime{11.1767}\\
4 & \prtime{8.60473}\\
5 & \prtime{16.8103}\\
6 & \prtime{39.919}\\
7 & \prtime{48.1031}\\
\midrule
 & \prtime{ 131.998320}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.255141}\\
3 & \prtime{1.32376}\\
4 & \prtime{0.686625}\\
5 & \prtime{2.25682}\\
6 & \prtime{6.55498}\\
7 & \prtime{28.6053}\\
\midrule
 & \prtime{ 41.111734}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b7 & \prtime{ 41.111734} & \prtime{0.255141} & \prtime{1.32376} & \prtime{0.686625} & \prtime{2.25682} & \prtime{6.55498} & \prtime{28.6053}&\prtime{ 94.890944}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.89421}\\
3 & \prtime{3.66931}\\
4 & \prtime{1.95726}\\
5 & \prtime{5.28645}\\
6 & \prtime{12.1633}\\
7 & \prtime{33.3894}\\
\midrule
 & \prtime{ 58.783904}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b7 & \prtime{ 58.783904} & \prtime{0.89421} & \prtime{3.66931} & \prtime{1.95726} & \prtime{5.28645} & \prtime{12.1633} & \prtime{33.3894}&\prtime{ 97.200787}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{6.81082}\\
3 & \prtime{5.72487}\\
4 & \prtime{3.41127}\\
5 & \prtime{9.785}\\
6 & \prtime{32.9625}\\
7 & \prtime{36.2072}\\
\midrule
 & \prtime{ 96.394597}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b7 & \prtime{ 96.394597} & \prtime{6.81082} & \prtime{5.72487} & \prtime{3.41127} & \prtime{9.785} & \prtime{32.9625} & \prtime{36.2072}&\prtime{ 97.516157}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.266374}\\
3 & \prtime{1.53925}\\
4 & \prtime{0.934853}\\
5 & \prtime{2.64598}\\
6 & \prtime{7.34317}\\
7 & \prtime{31.7772}\\
\midrule
 & \prtime{ 45.943758}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b7 & \prtime{ 45.943758} & \prtime{0.266374} & \prtime{1.53925} & \prtime{0.934853} & \prtime{2.64598} & \prtime{7.34317} & \prtime{31.7772}&\prtime{ 95.963929}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.13013}\\
3 & \prtime{5.34634}\\
4 & \prtime{2.66181}\\
5 & \prtime{5.81347}\\
6 & \prtime{13.133}\\
7 & \prtime{35.6651}\\
\midrule
 & \prtime{ 65.177606}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b7 & \prtime{ 65.177606} & \prtime{1.13013} & \prtime{5.34634} & \prtime{2.66181} & \prtime{5.81347} & \prtime{13.133} & \prtime{35.6651}&\prtime{ 97.237019}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.58786}\\
3 & \prtime{26.3621}\\
4 & \prtime{5.23718}\\
5 & \prtime{10.9441}\\
6 & \prtime{33.2802}\\
7 & \prtime{38.3686}\\
\midrule
 & \prtime{ 118.283642}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b7 & \prtime{ 118.283642} & \prtime{2.58786} & \prtime{26.3621} & \prtime{5.23718} & \prtime{10.9441} & \prtime{33.2802} & \prtime{38.3686}&\prtime{ 98.345933}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.270908}\\
3 & \prtime{1.62382}\\
4 & \prtime{1.60609}\\
5 & \prtime{3.97256}\\
6 & \prtime{22.32054}\\
\midrule
 & \prtime{ 30.169419}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 30.169419} & \prtime{0.270908} & \prtime{1.62382} & \prtime{1.60609} & \prtime{3.97256} & \prtime{22.32054}& &\prtime{ 99.745797}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.66203}\\
3 & \prtime{5.53759}\\
4 & \prtime{4.28535}\\
5 & \prtime{8.71838}\\
6 & \prtime{25.6841}\\
\midrule
 & \prtime{ 46.279553}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 46.279553} & \prtime{1.66203} & \prtime{5.53759} & \prtime{4.28535} & \prtime{8.71838} & \prtime{25.6841}& &\prtime{ 100.723252}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.06449}\\
3 & \prtime{11.1924}\\
4 & \prtime{7.89645}\\
5 & \prtime{16.0921}\\
6 & \prtime{45.3360}\\
\midrule
 & \prtime{ 85.982191}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.253182}\\
3 & \prtime{2.63447}\\
4 & \prtime{4.46554}\\
5 & \prtime{8.9165}\\
6 & \prtime{37.1299}\\
\midrule
 & \prtime{ 53.772756}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 53.772756} & \prtime{0.253182} & \prtime{2.63447} & \prtime{4.46554} & \prtime{8.9165} & \prtime{37.1299}& &\prtime{ 120.440930}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.44797}\\
3 & \prtime{8.34081}\\
4 & \prtime{9.20125}\\
5 & \prtime{16.4015}\\
6 & \prtime{45.0317}\\
\midrule
 & \prtime{ 80.797652}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 80.797652} & \prtime{1.44797} & \prtime{8.34081} & \prtime{9.20125} & \prtime{16.4015} & \prtime{45.0317}& &\prtime{ 121.949373}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{8.86444}\\
3 & \prtime{23.8674}\\
4 & \prtime{17.3906}\\
5 & \prtime{26.4906}\\
6 & \prtime{52.1099}\\
\midrule
 & \prtime{ 129.098626}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 129.098626} & \prtime{8.86444} & \prtime{23.8674} & \prtime{17.3906} & \prtime{26.4906} & \prtime{52.1099}& &\prtime{ 124.125904}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.242436}\\
3 & \prtime{1.28762}\\
4 & \prtime{0.652955}\\
5 & \prtime{2.18719}\\
6 & \prtime{15.41984}\\
\midrule
 & \prtime{ 20.163046}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 20.163046} & \prtime{0.242436} & \prtime{1.28762} & \prtime{0.652955} & \prtime{2.18719} & \prtime{15.41984}& &\prtime{ 92.066003}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.822967}\\
3 & \prtime{3.4688}\\
4 & \prtime{1.89245}\\
5 & \prtime{5.3112}\\
6 & \prtime{17.98466}\\
\midrule
 & \prtime{ 29.852865}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 29.852865} & \prtime{0.822967} & \prtime{3.4688} & \prtime{1.89245} & \prtime{5.3112} & \prtime{17.98466}& &\prtime{ 92.002232}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.52916}\\
3 & \prtime{5.69439}\\
4 & \prtime{3.2728}\\
5 & \prtime{9.69875}\\
6 & \prtime{35.5466}\\
\midrule
 & \prtime{ 56.130154}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 56.130154} & \prtime{1.52916} & \prtime{5.69439} & \prtime{3.2728} & \prtime{9.69875} & \prtime{35.5466}& &\prtime{ 92.873842}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.260198}\\
3 & \prtime{1.50968}\\
4 & \prtime{0.90431}\\
5 & \prtime{2.61266}\\
6 & \prtime{16.97001}\\
\midrule
 & \prtime{ 22.632914}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 22.632914} & \prtime{0.260198} & \prtime{1.50968} & \prtime{0.90431} & \prtime{2.61266} & \prtime{16.97001}& &\prtime{ 92.465611}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.05216}\\
3 & \prtime{4.47183}\\
4 & \prtime{2.58415}\\
5 & \prtime{5.96007}\\
6 & \prtime{20.28888}\\
\midrule
 & \prtime{ 34.729559}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 34.729559} & \prtime{1.05216} & \prtime{4.47183} & \prtime{2.58415} & \prtime{5.96007} & \prtime{20.28888}& &\prtime{ 92.958098}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.00264}\\
3 & \prtime{6.63048}\\
4 & \prtime{5.02969}\\
5 & \prtime{10.888}\\
6 & \prtime{37.00327}\\
\midrule
 & \prtime{ 61.956620}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b6 & \prtime{ 61.956620} & \prtime{2.00264} & \prtime{6.63048} & \prtime{5.02969} & \prtime{10.888} & \prtime{37.00327}& &\prtime{ 93.339009}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.27148}\\
3 & \prtime{1.59811}\\
4 & \prtime{1.61539}\\
5 & \prtime{59.15305}\\
\midrule
 & \prtime{ 62.732624}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 62.732624} & \prtime{0.27148} & \prtime{1.59811} & \prtime{1.61539} & \prtime{59.15305}& & &\prtime{ 413.647251}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.34538}\\
3 & \prtime{5.24484}\\
4 & \prtime{4.00893}\\
5 & \prtime{63.05405}\\
\midrule
 & \prtime{ 73.748066}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 73.748066} & \prtime{1.34538} & \prtime{5.24484} & \prtime{4.00893} & \prtime{63.05405}& & &\prtime{ 413.317587}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.80649}\\
3 & \prtime{10.0327}\\
4 & \prtime{9.51767}\\
5 & \prtime{103.83039}\\
\midrule
 & \prtime{ 126.295347}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.246182}\\
3 & \prtime{2.97244}\\
4 & \prtime{4.90341}\\
5 & \prtime{71.6891}\\
\midrule
 & \prtime{ 79.908146}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 79.908146} & \prtime{0.246182} & \prtime{2.97244} & \prtime{4.90341} & \prtime{71.6891}& & &\prtime{ 433.052108}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.53485}\\
3 & \prtime{8.4689}\\
4 & \prtime{8.97704}\\
5 & \prtime{77.4006}\\
\midrule
 & \prtime{ 96.477400}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 96.477400} & \prtime{1.53485} & \prtime{8.4689} & \prtime{8.97704} & \prtime{77.4006}& & &\prtime{ 433.096343}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{16.8061}\\
3 & \prtime{24.7066}\\
4 & \prtime{18.1666}\\
5 & \prtime{88.9409}\\
\midrule
 & \prtime{ 148.716003}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 148.716003} & \prtime{16.8061} & \prtime{24.7066} & \prtime{18.1666} & \prtime{88.9409}& & &\prtime{ 437.532701}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.238293}\\
3 & \prtime{1.20773}\\
4 & \prtime{0.642085}\\
5 & \prtime{53.32814}\\
\midrule
 & \prtime{ 55.512002}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 55.512002} & \prtime{0.238293} & \prtime{1.20773} & \prtime{0.642085} & \prtime{53.32814}& & &\prtime{ 386.033350}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.811659}\\
3 & \prtime{3.35967}\\
4 & \prtime{1.87515}\\
5 & \prtime{56.44442}\\
\midrule
 & \prtime{ 62.593866}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 62.593866} & \prtime{0.811659} & \prtime{3.35967} & \prtime{1.87515} & \prtime{56.44442}& & &\prtime{ 386.204980}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.38797}\\
3 & \prtime{5.0869}\\
4 & \prtime{4.43136}\\
5 & \prtime{91.58621}\\
\midrule
 & \prtime{ 102.589177}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 102.589177} & \prtime{1.38797} & \prtime{5.0869} & \prtime{4.43136} & \prtime{91.58621}& & &\prtime{ 386.727365}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.2563}\\
3 & \prtime{1.42238}\\
4 & \prtime{0.89416}\\
5 & \prtime{54.99702}\\
\midrule
 & \prtime{ 57.665505}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 57.665505} & \prtime{0.2563} & \prtime{1.42238} & \prtime{0.89416} & \prtime{54.99702}& & &\prtime{ 403.923293}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.07903}\\
3 & \prtime{5.57787}\\
4 & \prtime{2.5492}\\
5 & \prtime{58.2016}\\
\midrule
 & \prtime{ 67.502707}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 67.502707} & \prtime{1.07903} & \prtime{5.57787} & \prtime{2.5492} & \prtime{58.2016}& & &\prtime{ 404.546159}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{7.17079}\\
3 & \prtime{6.16096}\\
4 & \prtime{6.34236}\\
5 & \prtime{96.97989}\\
\midrule
 & \prtime{ 116.752593}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b5 & \prtime{ 116.752593} & \prtime{7.17079} & \prtime{6.16096} & \prtime{6.34236} & \prtime{96.97989}& & &\prtime{ 407.681727}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.225769}\\
3 & \prtime{1.62959}\\
4 & \prtime{621.8573}\\
\midrule
 & \prtime{ 623.736159}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 623.736159} & \prtime{0.225769} & \prtime{1.62959} & \prtime{621.8573}& & & &\prtime{ 1745.297034}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.39798}\\
3 & \prtime{5.20661}\\
4 & \prtime{630.690}\\
\midrule
 & \prtime{ 637.317818}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 637.317818} & \prtime{1.39798} & \prtime{5.20661} & \prtime{630.690}& & & &\prtime{ 1769.186807}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.63504}\\
3 & \prtime{11.493}\\
4 & \prtime{970.9873}\\
\midrule
 & \prtime{ 987.142215}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.241454}\\
3 & \prtime{2.96858}\\
4 & \prtime{623.0363}\\
\midrule
 & \prtime{ 626.270147}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 626.270147} & \prtime{0.241454} & \prtime{2.96858} & \prtime{623.0363}& & & &\prtime{ 1801.948392}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.31436}\\
3 & \prtime{7.75431}\\
4 & \prtime{634.5666}\\
\midrule
 & \prtime{ 643.658793}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 643.658793} & \prtime{1.31436} & \prtime{7.75431} & \prtime{634.5666}& & & &\prtime{ 1807.634828}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{9.11652}\\
3 & \prtime{16.4107}\\
4 & \prtime{667.0287}\\
\midrule
 & \prtime{ 692.579622}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 692.579622} & \prtime{9.11652} & \prtime{16.4107} & \prtime{667.0287}& & & &\prtime{ 1803.654252}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.243659}\\
3 & \prtime{1.23213}\\
4 & \prtime{623.995}\\
\midrule
 & \prtime{ 625.493686}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 625.493686} & \prtime{0.243659} & \prtime{1.23213} & \prtime{623.995}& & & &\prtime{ 1708.951620}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.901068}\\
3 & \prtime{4.72759}\\
4 & \prtime{629.9915}\\
\midrule
 & \prtime{ 635.644146}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 635.644146} & \prtime{0.901068} & \prtime{4.72759} & \prtime{629.9915}& & & &\prtime{ 1700.362754}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.24759}\\
3 & \prtime{6.52443}\\
4 & \prtime{936.8087}\\
\midrule
 & \prtime{ 944.604943}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 944.604943} & \prtime{1.24759} & \prtime{6.52443} & \prtime{936.8087}& & & &\prtime{ 1736.184406}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.258571}\\
3 & \prtime{1.46702}\\
4 & \prtime{616.2369}\\
\midrule
 & \prtime{ 617.987481}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 617.987481} & \prtime{0.258571} & \prtime{1.46702} & \prtime{616.2369}& & & &\prtime{ 1712.351279}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.05766}\\
3 & \prtime{5.055}\\
4 & \prtime{624.8565}\\
\midrule
 & \prtime{ 630.992773}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 630.992773} & \prtime{1.05766} & \prtime{5.055} & \prtime{624.8565}& & & &\prtime{ 1737.350074}\\


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.69503}\\
3 & \prtime{8.40979}\\
4 & \prtime{951.4592}\\
\midrule
 & \prtime{ 961.590144}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep3top4sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs3t4b4 & \prtime{ 961.590144} & \prtime{1.69503} & \prtime{8.40979} & \prtime{951.4592}& & & &\prtime{ 1728.624314}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{9.8055}\\
3 & \prtime{13.7105}\\
4 & \prtime{15.0278}\\
5 & \prtime{22.6521}\\
6 & \prtime{36.1841}\\
7 & \prtime{49.1296}\\
\midrule
 & \prtime{ 148.047420}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b7 & \prtime{ 148.047420} & \prtime{9.8055} & \prtime{13.7105} & \prtime{15.0278} & \prtime{22.6521} & \prtime{36.1841} & \prtime{49.1296}&\prtime{ 100.945815}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.43986}\\
3 & \prtime{12.0317}\\
4 & \prtime{6.49785}\\
5 & \prtime{13.7951}\\
6 & \prtime{28.4958}\\
7 & \prtime{36.0657}\\
\midrule
 & \prtime{ 103.819122}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b7 & \prtime{ 103.819122} & \prtime{5.43986} & \prtime{12.0317} & \prtime{6.49785} & \prtime{13.7951} & \prtime{28.4958} & \prtime{36.0657}&\prtime{ 98.408168}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{15.6772}\\
3 & \prtime{7.42501}\\
4 & \prtime{9.77551}\\
5 & \prtime{14.9102}\\
6 & \prtime{29.3571}\\
7 & \prtime{37.7394}\\
\midrule
 & \prtime{ 116.347208}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b7 & \prtime{ 116.347208} & \prtime{15.6772} & \prtime{7.42501} & \prtime{9.77551} & \prtime{14.9102} & \prtime{29.3571} & \prtime{37.7394}&\prtime{ 99.497578}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{10.2794}\\
3 & \prtime{13.7994}\\
4 & \prtime{13.9003}\\
5 & \prtime{21.9919}\\
6 & \prtime{46.8469}\\
\midrule
 & \prtime{ 107.236840}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b6 & \prtime{ 107.236840} & \prtime{10.2794} & \prtime{13.7994} & \prtime{13.9003} & \prtime{21.9919} & \prtime{46.8469}& &\prtime{ 101.096668}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{19.374}\\
3 & \prtime{31.0892}\\
4 & \prtime{27.1988}\\
5 & \prtime{33.6489}\\
6 & \prtime{54.5359}\\
\midrule
 & \prtime{ 166.234635}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b6 & \prtime{ 166.234635} & \prtime{19.374} & \prtime{31.0892} & \prtime{27.1988} & \prtime{33.6489} & \prtime{54.5359}& &\prtime{ 120.980441}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{7.87176}\\
3 & \prtime{5.09033}\\
4 & \prtime{6.14596}\\
5 & \prtime{13.6199}\\
6 & \prtime{33.60154}\\
\midrule
 & \prtime{ 66.730419}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b6 & \prtime{ 66.730419} & \prtime{7.87176} & \prtime{5.09033} & \prtime{6.14596} & \prtime{13.6199} & \prtime{33.60154}& &\prtime{ 93.210242}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.15513}\\
3 & \prtime{7.06087}\\
4 & \prtime{9.19398}\\
5 & \prtime{14.927}\\
6 & \prtime{35.98422}\\
\midrule
 & \prtime{ 72.715642}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b6 & \prtime{ 72.715642} & \prtime{5.15513} & \prtime{7.06087} & \prtime{9.19398} & \prtime{14.927} & \prtime{35.98422}& &\prtime{ 93.119649}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{8.69509}\\
3 & \prtime{11.9822}\\
4 & \prtime{17.0533}\\
5 & \prtime{150.8994}\\
\midrule
 & \prtime{ 188.736103}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b5 & \prtime{ 188.736103} & \prtime{8.69509} & \prtime{11.9822} & \prtime{17.0533} & \prtime{150.8994}& & &\prtime{ 406.880008}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{19.0812}\\
3 & \prtime{23.6681}\\
4 & \prtime{27.6406}\\
5 & \prtime{124.7149}\\
\midrule
 & \prtime{ 195.210893}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b5 & \prtime{ 195.210893} & \prtime{19.0812} & \prtime{23.6681} & \prtime{27.6406} & \prtime{124.7149}& & &\prtime{ 434.231284}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.92795}\\
3 & \prtime{4.89267}\\
4 & \prtime{8.64847}\\
5 & \prtime{128.00315}\\
\midrule
 & \prtime{ 144.572006}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b5 & \prtime{ 144.572006} & \prtime{2.92795} & \prtime{4.89267} & \prtime{8.64847} & \prtime{128.00315}& & &\prtime{ 387.226726}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{16.4956}\\
3 & \prtime{6.72829}\\
4 & \prtime{11.9775}\\
5 & \prtime{141.26771}\\
\midrule
 & \prtime{ 176.575501}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b5 & \prtime{ 176.575501} & \prtime{16.4956} & \prtime{6.72829} & \prtime{11.9775} & \prtime{141.26771}& & &\prtime{ 398.364826}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{8.25943}\\
3 & \prtime{16.86}\\
4 & \prtime{1780.8586}\\
\midrule
 & \prtime{ 1806.004314}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b4 & \prtime{ 1806.004314} & \prtime{8.25943} & \prtime{16.86} & \prtime{1780.8586}& & & &\prtime{ 1722.133507}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{12.559}\\
3 & \prtime{25.7199}\\
4 & \prtime{1332.7387}\\
\midrule
 & \prtime{ 1371.043185}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b4 & \prtime{ 1371.043185} & \prtime{12.559} & \prtime{25.7199} & \prtime{1332.7387}& & & &\prtime{ 1775.582358}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.84933}\\
3 & \prtime{7.33553}\\
4 & \prtime{1696.8508}\\
\midrule
 & \prtime{ 1707.059116}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b4 & \prtime{ 1707.059116} & \prtime{2.84933} & \prtime{7.33553} & \prtime{1696.8508}& & & &\prtime{ 1708.795450}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.54255}\\
3 & \prtime{10.2283}\\
4 & \prtime{1734.3415}\\
\midrule
 & \prtime{ 1749.138814}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top2sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t2b4 & \prtime{ 1749.138814} & \prtime{4.54255} & \prtime{10.2283} & \prtime{1734.3415}& & & &\prtime{ 1692.680608}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{3.33812}\\
3 & \prtime{13.3888}\\
4 & \prtime{14.7947}\\
5 & \prtime{22.6533}\\
6 & \prtime{35.1991}\\
7 & \prtime{46.4251}\\
\midrule
 & \prtime{ 137.250256}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b7 & \prtime{ 137.250256} & \prtime{3.33812} & \prtime{13.3888} & \prtime{14.7947} & \prtime{22.6533} & \prtime{35.1991} & \prtime{46.4251}&\prtime{ 101.984524}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.8585}\\
3 & \prtime{11.9136}\\
4 & \prtime{6.35476}\\
5 & \prtime{13.6153}\\
6 & \prtime{28.1545}\\
7 & \prtime{35.5702}\\
\midrule
 & \prtime{ 99.903181}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b7 & \prtime{ 99.903181} & \prtime{2.8585} & \prtime{11.9136} & \prtime{6.35476} & \prtime{13.6153} & \prtime{28.1545} & \prtime{35.5702}&\prtime{ 95.289979}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{13.2692}\\
3 & \prtime{7.41176}\\
4 & \prtime{9.77254}\\
5 & \prtime{14.9232}\\
6 & \prtime{29.1187}\\
7 & \prtime{37.8489}\\
\midrule
 & \prtime{ 113.775208}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b7 & \prtime{ 113.775208} & \prtime{13.2692} & \prtime{7.41176} & \prtime{9.77254} & \prtime{14.9232} & \prtime{29.1187} & \prtime{37.8489}&\prtime{ 99.156940}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.4062}\\
3 & \prtime{13.7524}\\
4 & \prtime{13.8781}\\
5 & \prtime{22.0019}\\
6 & \prtime{44.4458}\\
\midrule
 & \prtime{ 98.873479}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b6 & \prtime{ 98.873479} & \prtime{4.4062} & \prtime{13.7524} & \prtime{13.8781} & \prtime{22.0019} & \prtime{44.4458}& &\prtime{ 101.992438}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{11.3745}\\
3 & \prtime{31.2175}\\
4 & \prtime{27.2842}\\
5 & \prtime{33.7789}\\
6 & \prtime{54.4749}\\
\midrule
 & \prtime{ 158.547523}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b6 & \prtime{ 158.547523} & \prtime{11.3745} & \prtime{31.2175} & \prtime{27.2842} & \prtime{33.7789} & \prtime{54.4749}& &\prtime{ 123.525612}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.8908}\\
3 & \prtime{5.11529}\\
4 & \prtime{6.14218}\\
5 & \prtime{13.6091}\\
6 & \prtime{33.41491}\\
\midrule
 & \prtime{ 64.552321}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b6 & \prtime{ 64.552321} & \prtime{5.8908} & \prtime{5.11529} & \prtime{6.14218} & \prtime{13.6091} & \prtime{33.41491}& &\prtime{ 92.929024}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.98566}\\
3 & \prtime{7.06599}\\
4 & \prtime{9.24913}\\
5 & \prtime{14.9281}\\
6 & \prtime{35.47236}\\
\midrule
 & \prtime{ 69.092076}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b6 & \prtime{ 69.092076} & \prtime{1.98566} & \prtime{7.06599} & \prtime{9.24913} & \prtime{14.9281} & \prtime{35.47236}& &\prtime{ 94.093496}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.77548}\\
3 & \prtime{12.0386}\\
4 & \prtime{17.0947}\\
5 & \prtime{151.65395}\\
\midrule
 & \prtime{ 183.661388}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b5 & \prtime{ 183.661388} & \prtime{2.77548} & \prtime{12.0386} & \prtime{17.0947} & \prtime{151.65395}& & &\prtime{ 411.997391}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{11.0936}\\
3 & \prtime{24.4828}\\
4 & \prtime{27.5381}\\
5 & \prtime{124.620}\\
\midrule
 & \prtime{ 187.837372}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b5 & \prtime{ 187.837372} & \prtime{11.0936} & \prtime{24.4828} & \prtime{27.5381} & \prtime{124.620}& & &\prtime{ 435.353708}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.28394}\\
3 & \prtime{4.91389}\\
4 & \prtime{8.64246}\\
5 & \prtime{128.59944}\\
\midrule
 & \prtime{ 143.537512}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b5 & \prtime{ 143.537512} & \prtime{1.28394} & \prtime{4.91389} & \prtime{8.64246} & \prtime{128.59944}& & &\prtime{ 387.563750}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{14.3577}\\
3 & \prtime{6.74999}\\
4 & \prtime{12.0312}\\
5 & \prtime{142.07005}\\
\midrule
 & \prtime{ 175.308075}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b5 & \prtime{ 175.308075} & \prtime{14.3577} & \prtime{6.74999} & \prtime{12.0312} & \prtime{142.07005}& & &\prtime{ 405.136408}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.91662}\\
3 & \prtime{16.93}\\
4 & \prtime{1784.6699}\\
\midrule
 & \prtime{ 1804.540190}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b4 & \prtime{ 1804.540190} & \prtime{2.91662} & \prtime{16.93} & \prtime{1784.6699}& & & &\prtime{ 1815.807099}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.5809}\\
3 & \prtime{25.352}\\
4 & \prtime{1336.2334}\\
\midrule
 & \prtime{ 1366.188190}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b4 & \prtime{ 1366.188190} & \prtime{4.5809} & \prtime{25.352} & \prtime{1336.2334}& & & &\prtime{ 1874.846287}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.34503}\\
3 & \prtime{7.35598}\\
4 & \prtime{1697.6723}\\
\midrule
 & \prtime{ 1706.400852}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b4 & \prtime{ 1706.400852} & \prtime{1.34503} & \prtime{7.35598} & \prtime{1697.6723}& & & &\prtime{ 1757.211895}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.75127}\\
3 & \prtime{10.2791}\\
4 & \prtime{1741.5336}\\
\midrule
 & \prtime{ 1753.589846}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top3sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t3b4 & \prtime{ 1753.589846} & \prtime{1.75127} & \prtime{10.2791} & \prtime{1741.5336}& & & &\prtime{ 1752.943193}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{3.47658}\\
3 & \prtime{11.0098}\\
4 & \prtime{15.0126}\\
5 & \prtime{22.9051}\\
6 & \prtime{35.8178}\\
7 & \prtime{48.4105}\\
\midrule
 & \prtime{ 138.136029}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b7 & \prtime{ 138.136029} & \prtime{3.47658} & \prtime{11.0098} & \prtime{15.0126} & \prtime{22.9051} & \prtime{35.8178} & \prtime{48.4105}&\prtime{ 103.034267}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.81615}\\
3 & \prtime{15.7363}\\
4 & \prtime{6.43999}\\
5 & \prtime{13.7357}\\
6 & \prtime{29.0062}\\
7 & \prtime{36.5755}\\
\midrule
 & \prtime{ 104.835304}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b7 & \prtime{ 104.835304} & \prtime{1.81615} & \prtime{15.7363} & \prtime{6.43999} & \prtime{13.7357} & \prtime{29.0062} & \prtime{36.5755}&\prtime{ 98.467237}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{13.4314}\\
3 & \prtime{6.81157}\\
4 & \prtime{9.82354}\\
5 & \prtime{15.1356}\\
6 & \prtime{29.4836}\\
7 & \prtime{38.0467}\\
\midrule
 & \prtime{ 114.182887}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b7 & \prtime{ 114.182887} & \prtime{13.4314} & \prtime{6.81157} & \prtime{9.82354} & \prtime{15.1356} & \prtime{29.4836} & \prtime{38.0467}&\prtime{ 98.205411}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{3.3767}\\
3 & \prtime{11.5522}\\
4 & \prtime{13.9153}\\
5 & \prtime{21.9448}\\
6 & \prtime{44.9918}\\
\midrule
 & \prtime{ 96.175432}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b6 & \prtime{ 96.175432} & \prtime{3.3767} & \prtime{11.5522} & \prtime{13.9153} & \prtime{21.9448} & \prtime{44.9918}& &\prtime{ 101.285350}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{12.9859}\\
3 & \prtime{27.3084}\\
4 & \prtime{28.5321}\\
5 & \prtime{34.5819}\\
6 & \prtime{54.1526}\\
\midrule
 & \prtime{ 157.947305}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b6 & \prtime{ 157.947305} & \prtime{12.9859} & \prtime{27.3084} & \prtime{28.5321} & \prtime{34.5819} & \prtime{54.1526}& &\prtime{ 124.155130}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.8019}\\
3 & \prtime{5.37487}\\
4 & \prtime{6.16274}\\
5 & \prtime{13.6953}\\
6 & \prtime{33.43053}\\
\midrule
 & \prtime{ 64.866134}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b6 & \prtime{ 64.866134} & \prtime{5.8019} & \prtime{5.37487} & \prtime{6.16274} & \prtime{13.6953} & \prtime{33.43053}& &\prtime{ 92.973842}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.96585}\\
3 & \prtime{6.65312}\\
4 & \prtime{9.25193}\\
5 & \prtime{15.0416}\\
6 & \prtime{35.30841}\\
\midrule
 & \prtime{ 68.616876}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b6 & \prtime{ 68.616876} & \prtime{1.96585} & \prtime{6.65312} & \prtime{9.25193} & \prtime{15.0416} & \prtime{35.30841}& &\prtime{ 93.698033}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.78283}\\
3 & \prtime{9.56609}\\
4 & \prtime{17.1011}\\
5 & \prtime{151.53875}\\
\midrule
 & \prtime{ 181.095710}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b5 & \prtime{ 181.095710} & \prtime{2.78283} & \prtime{9.56609} & \prtime{17.1011} & \prtime{151.53875}& & &\prtime{ 423.288222}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.17318}\\
3 & \prtime{17.5562}\\
4 & \prtime{27.6918}\\
5 & \prtime{124.8121}\\
\midrule
 & \prtime{ 175.328868}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b5 & \prtime{ 175.328868} & \prtime{5.17318} & \prtime{17.5562} & \prtime{27.6918} & \prtime{124.8121}& & &\prtime{ 444.315605}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.27096}\\
3 & \prtime{5.01424}\\
4 & \prtime{8.63517}\\
5 & \prtime{128.5267}\\
\midrule
 & \prtime{ 143.545466}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b5 & \prtime{ 143.545466} & \prtime{1.27096} & \prtime{5.01424} & \prtime{8.63517} & \prtime{128.5267}& & &\prtime{ 397.098494}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{14.1255}\\
3 & \prtime{6.12801}\\
4 & \prtime{12.0251}\\
5 & \prtime{141.86699}\\
\midrule
 & \prtime{ 174.243856}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b5 & \prtime{ 174.243856} & \prtime{14.1255} & \prtime{6.12801} & \prtime{12.0251} & \prtime{141.86699}& & &\prtime{ 414.986781}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.86118}\\
3 & \prtime{11.6246}\\
4 & \prtime{1779.9486}\\
\midrule
 & \prtime{ 1794.455805}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b4 & \prtime{ 1794.455805} & \prtime{2.86118} & \prtime{11.6246} & \prtime{1779.9486}& & & &\prtime{ 1783.298649}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.83921}\\
3 & \prtime{18.9538}\\
4 & \prtime{1335.9601}\\
\midrule
 & \prtime{ 1359.775787}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b4 & \prtime{ 1359.775787} & \prtime{4.83921} & \prtime{18.9538} & \prtime{1335.9601}& & & &\prtime{ 1819.324209}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.2323}\\
3 & \prtime{6.47407}\\
4 & \prtime{1701.3317}\\
\midrule
 & \prtime{ 1709.058658}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b4 & \prtime{ 1709.058658} & \prtime{1.2323} & \prtime{6.47407} & \prtime{1701.3317}& & & &\prtime{ 1788.939368}\\


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.74552}\\
3 & \prtime{8.08932}\\
4 & \prtime{1737.4232}\\
\midrule
 & \prtime{ 1747.286456}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsep6top4sub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
nIFMMs6t4b4 & \prtime{ 1747.286456} & \prtime{1.74552} & \prtime{8.08932} & \prtime{1737.4232}& & & &\prtime{ 1752.233408}\\


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.262826}\\
3 & \prtime{1.53517}\\
4 & \prtime{5.92341}\\
5 & \prtime{19.8286}\\
6 & \prtime{51.3467}\\
7 & \prtime{102.6964}\\
\midrule
 & \prtime{ 183.007394}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 183.007394} & \prtime{0.262826} & \prtime{1.53517} & \prtime{5.92341} & \prtime{19.8286} & \prtime{51.3467} & \prtime{102.6964}&\prtime{ 97.853928}\\


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.16963}\\
3 & \prtime{5.2784}\\
4 & \prtime{17.5053}\\
5 & \prtime{51.1043}\\
6 & \prtime{104.073}\\
7 & \prtime{119.1763}\\
\midrule
 & \prtime{ 299.761779}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 299.761779} & \prtime{1.16963} & \prtime{5.2784} & \prtime{17.5053} & \prtime{51.1043} & \prtime{104.073} & \prtime{119.1763}&\prtime{ 101.932577}\\


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{3.16257}\\
3 & \prtime{12.252}\\
4 & \prtime{26.6193}\\
5 & \prtime{88.7144}\\
6 & \prtime{195.02}\\
7 & \prtime{122.4348}\\
\midrule
 & \prtime{ 449.689778}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 449.689778} & \prtime{3.16257} & \prtime{12.252} & \prtime{26.6193} & \prtime{88.7144} & \prtime{195.02} & \prtime{122.4348}&\prtime{ 102.171225}\\


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.239148}\\
3 & \prtime{1.21423}\\
4 & \prtime{4.62261}\\
5 & \prtime{17.1222}\\
6 & \prtime{49.3203}\\
7 & \prtime{95.3267}\\
\midrule
 & \prtime{ 169.265063}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 169.265063} & \prtime{0.239148} & \prtime{1.21423} & \prtime{4.62261} & \prtime{17.1222} & \prtime{49.3203} & \prtime{95.3267}&\prtime{ 95.810019}\\


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.80712}\\
3 & \prtime{3.34236}\\
4 & \prtime{11.3327}\\
5 & \prtime{39.9402}\\
6 & \prtime{94.82}\\
7 & \prtime{103.2756}\\
\midrule
 & \prtime{ 254.980375}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 254.980375} & \prtime{0.80712} & \prtime{3.34236} & \prtime{11.3327} & \prtime{39.9402} & \prtime{94.82} & \prtime{103.2756}&\prtime{ 98.727030}\\


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.09204}\\
3 & \prtime{5.01157}\\
4 & \prtime{17.1039}\\
5 & \prtime{62.2334}\\
6 & \prtime{168.913}\\
7 & \prtime{104.0629}\\
\midrule
 & \prtime{ 363.857506}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 363.857506} & \prtime{5.09204} & \prtime{5.01157} & \prtime{17.1039} & \prtime{62.2334} & \prtime{168.913} & \prtime{104.0629}&\prtime{ 97.676756}\\


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.257217}\\
3 & \prtime{1.49788}\\
4 & \prtime{5.209}\\
5 & \prtime{17.9487}\\
6 & \prtime{50.5848}\\
7 & \prtime{98.9788}\\
\midrule
 & \prtime{ 175.906538}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 175.906538} & \prtime{0.257217} & \prtime{1.49788} & \prtime{5.209} & \prtime{17.9487} & \prtime{50.5848} & \prtime{98.9788}&\prtime{ 97.977486}\\


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.06561}\\
3 & \prtime{5.70188}\\
4 & \prtime{14.2008}\\
5 & \prtime{40.9211}\\
6 & \prtime{94.5264}\\
7 & \prtime{103.3763}\\
\midrule
 & \prtime{ 261.257259}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 261.257259} & \prtime{1.06561} & \prtime{5.70188} & \prtime{14.2008} & \prtime{40.9211} & \prtime{94.5264} & \prtime{103.3763}&\prtime{ 99.153868}\\


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.065}\\
3 & \prtime{6.434}\\
4 & \prtime{20.8802}\\
5 & \prtime{64.9983}\\
6 & \prtime{168.419}\\
7 & \prtime{106.7683}\\
\midrule
 & \prtime{ 371.008166}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub0-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb7 & \prtime{ 371.008166} & \prtime{2.065} & \prtime{6.434} & \prtime{20.8802} & \prtime{64.9983} & \prtime{168.419} & \prtime{106.7683}&\prtime{ 96.165879}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.270417}\\
3 & \prtime{1.61227}\\
4 & \prtime{6.24022}\\
5 & \prtime{21.264}\\
6 & \prtime{107.94828}\\
\midrule
 & \prtime{ 137.730638}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 137.730638} & \prtime{0.270417} & \prtime{1.61227} & \prtime{6.24022} & \prtime{21.264} & \prtime{107.94828}& &\prtime{ 100.612053}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.31506}\\
3 & \prtime{5.3687}\\
4 & \prtime{18.2475}\\
5 & \prtime{53.1149}\\
6 & \prtime{129.3903}\\
\midrule
 & \prtime{ 207.823370}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 207.823370} & \prtime{1.31506} & \prtime{5.3687} & \prtime{18.2475} & \prtime{53.1149} & \prtime{129.3903}& &\prtime{ 102.177019}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.99025}\\
3 & \prtime{14.4825}\\
4 & \prtime{25.7526}\\
5 & \prtime{86.642}\\
6 & \prtime{209.8266}\\
\midrule
 & \prtime{ 340.097770}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 340.097770} & \prtime{2.99025} & \prtime{14.4825} & \prtime{25.7526} & \prtime{86.642} & \prtime{209.8266}& &\prtime{ 101.386314}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.239521}\\
3 & \prtime{2.9506}\\
4 & \prtime{9.16092}\\
5 & \prtime{26.3219}\\
6 & \prtime{123.1283}\\
\midrule
 & \prtime{ 162.223708}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 162.223708} & \prtime{0.239521} & \prtime{2.9506} & \prtime{9.16092} & \prtime{26.3219} & \prtime{123.1283}& &\prtime{ 120.842558}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.24384}\\
3 & \prtime{8.18315}\\
4 & \prtime{25.0453}\\
5 & \prtime{69.4075}\\
6 & \prtime{150.3478}\\
\midrule
 & \prtime{ 254.616786}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 254.616786} & \prtime{1.24384} & \prtime{8.18315} & \prtime{25.0453} & \prtime{69.4075} & \prtime{150.3478}& &\prtime{ 124.445683}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{8.72562}\\
3 & \prtime{16.382}\\
4 & \prtime{41.1341}\\
5 & \prtime{102.663}\\
6 & \prtime{167.0712}\\
\midrule
 & \prtime{ 336.366946}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 336.366946} & \prtime{8.72562} & \prtime{16.382} & \prtime{41.1341} & \prtime{102.663} & \prtime{167.0712}& &\prtime{ 123.815504}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.238408}\\
3 & \prtime{1.22134}\\
4 & \prtime{4.70656}\\
5 & \prtime{17.6862}\\
6 & \prtime{100.12213}\\
\midrule
 & \prtime{ 124.347438}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 124.347438} & \prtime{0.238408} & \prtime{1.22134} & \prtime{4.70656} & \prtime{17.6862} & \prtime{100.12213}& &\prtime{ 93.720154}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.795363}\\
3 & \prtime{3.25957}\\
4 & \prtime{11.1818}\\
5 & \prtime{40.4784}\\
6 & \prtime{113.57741}\\
\midrule
 & \prtime{ 169.678745}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 169.678745} & \prtime{0.795363} & \prtime{3.25957} & \prtime{11.1818} & \prtime{40.4784} & \prtime{113.57741}& &\prtime{ 92.090634}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.3338}\\
3 & \prtime{6.13583}\\
4 & \prtime{17.0559}\\
5 & \prtime{66.8193}\\
6 & \prtime{188.12366}\\
\midrule
 & \prtime{ 279.876724}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 279.876724} & \prtime{1.3338} & \prtime{6.13583} & \prtime{17.0559} & \prtime{66.8193} & \prtime{188.12366}& &\prtime{ 92.944932}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.254654}\\
3 & \prtime{1.47362}\\
4 & \prtime{5.26407}\\
5 & \prtime{18.0674}\\
6 & \prtime{101.1096}\\
\midrule
 & \prtime{ 126.543522}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 126.543522} & \prtime{0.254654} & \prtime{1.47362} & \prtime{5.26407} & \prtime{18.0674} & \prtime{101.1096}& &\prtime{ 93.093843}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.02161}\\
3 & \prtime{4.76295}\\
4 & \prtime{13.6756}\\
5 & \prtime{41.9292}\\
6 & \prtime{115.42351}\\
\midrule
 & \prtime{ 177.199450}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 177.199450} & \prtime{1.02161} & \prtime{4.76295} & \prtime{13.6756} & \prtime{41.9292} & \prtime{115.42351}& &\prtime{ 93.140092}\\


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.73142}\\
3 & \prtime{6.13516}\\
4 & \prtime{20.8907}\\
5 & \prtime{70.2385}\\
6 & \prtime{189.78006}\\
\midrule
 & \prtime{ 290.186282}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub1-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb6 & \prtime{ 290.186282} & \prtime{2.73142} & \prtime{6.13516} & \prtime{20.8907} & \prtime{70.2385} & \prtime{189.78006}& &\prtime{ 93.584054}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.26949}\\
3 & \prtime{1.64005}\\
4 & \prtime{6.23253}\\
5 & \prtime{191.36177}\\
\midrule
 & \prtime{ 199.609830}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 199.609830} & \prtime{0.26949} & \prtime{1.64005} & \prtime{6.23253} & \prtime{191.36177}& & &\prtime{ 450.488898}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.60153}\\
3 & \prtime{5.21723}\\
4 & \prtime{17.9173}\\
5 & \prtime{208.56074}\\
\midrule
 & \prtime{ 233.405584}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 233.405584} & \prtime{1.60153} & \prtime{5.21723} & \prtime{17.9173} & \prtime{208.56074}& & &\prtime{ 443.894174}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.80582}\\
3 & \prtime{9.97675}\\
4 & \prtime{32.4961}\\
5 & \prtime{442.29456}\\
\midrule
 & \prtime{ 487.696048}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 487.696048} & \prtime{2.80582} & \prtime{9.97675} & \prtime{32.4961} & \prtime{442.29456}& & &\prtime{ 442.707179}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.243747}\\
3 & \prtime{3.1158}\\
4 & \prtime{10.0795}\\
5 & \prtime{202.5974}\\
\midrule
 & \prtime{ 216.146636}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 216.146636} & \prtime{0.243747} & \prtime{3.1158} & \prtime{10.0795} & \prtime{202.5974}& & &\prtime{ 472.341468}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.24415}\\
3 & \prtime{8.13334}\\
4 & \prtime{23.7201}\\
5 & \prtime{224.7955}\\
\midrule
 & \prtime{ 257.994451}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 257.994451} & \prtime{1.24415} & \prtime{8.13334} & \prtime{23.7201} & \prtime{224.7955}& & &\prtime{ 460.700994}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{18.1765}\\
3 & \prtime{17.1251}\\
4 & \prtime{41.3815}\\
5 & \prtime{275.1075}\\
\midrule
 & \prtime{ 351.901357}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 351.901357} & \prtime{18.1765} & \prtime{17.1251} & \prtime{41.3815} & \prtime{275.1075}& & &\prtime{ 457.413696}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.238003}\\
3 & \prtime{1.2151}\\
4 & \prtime{4.66833}\\
5 & \prtime{184.04895}\\
\midrule
 & \prtime{ 190.270779}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 190.270779} & \prtime{0.238003} & \prtime{1.2151} & \prtime{4.66833} & \prtime{184.04895}& & &\prtime{ 413.344841}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.794349}\\
3 & \prtime{3.21764}\\
4 & \prtime{11.2031}\\
5 & \prtime{198.40316}\\
\midrule
 & \prtime{ 213.719197}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 213.719197} & \prtime{0.794349} & \prtime{3.21764} & \prtime{11.2031} & \prtime{198.40316}& & &\prtime{ 415.377531}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{5.16698}\\
3 & \prtime{5.08148}\\
4 & \prtime{21.7024}\\
5 & \prtime{336.41071}\\
\midrule
 & \prtime{ 368.468279}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 368.468279} & \prtime{5.16698} & \prtime{5.08148} & \prtime{21.7024} & \prtime{336.41071}& & &\prtime{ 413.833751}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.252695}\\
3 & \prtime{1.42893}\\
4 & \prtime{5.28581}\\
5 & \prtime{187.0898}\\
\midrule
 & \prtime{ 194.157764}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 194.157764} & \prtime{0.252695} & \prtime{1.42893} & \prtime{5.28581} & \prtime{187.0898}& & &\prtime{ 438.284576}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.051}\\
3 & \prtime{5.18139}\\
4 & \prtime{13.6116}\\
5 & \prtime{202.18442}\\
\midrule
 & \prtime{ 222.130159}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 222.130159} & \prtime{1.051} & \prtime{5.18139} & \prtime{13.6116} & \prtime{202.18442}& & &\prtime{ 439.663428}\\


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.36794}\\
3 & \prtime{6.25227}\\
4 & \prtime{26.2436}\\
5 & \prtime{399.69027}\\
\midrule
 & \prtime{ 436.675023}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub2-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb5 & \prtime{ 436.675023} & \prtime{4.36794} & \prtime{6.25227} & \prtime{26.2436} & \prtime{399.69027}& & &\prtime{ 425.759342}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.222015}\\
3 & \prtime{1.61167}\\
4 & \prtime{1063.2184}\\
\midrule
 & \prtime{ 1065.074147}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1065.074147} & \prtime{0.222015} & \prtime{1.61167} & \prtime{1063.2184}& & & &\prtime{ 1829.122600}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.46956}\\
3 & \prtime{5.30575}\\
4 & \prtime{1080.7647}\\
\midrule
 & \prtime{ 1087.566976}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1087.566976} & \prtime{1.46956} & \prtime{5.30575} & \prtime{1080.7647}& & & &\prtime{ 1780.499518}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{2.8659}\\
3 & \prtime{12.3049}\\
4 & \prtime{1521.0635}\\
\midrule
 & \prtime{ 1536.263757}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk16.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1536.263757} & \prtime{2.8659} & \prtime{12.3049} & \prtime{1521.0635}& & & &\prtime{ 1860.872657}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.2426}\\
3 & \prtime{3.21419}\\
4 & \prtime{1049.1886}\\
\midrule
 & \prtime{ 1052.672904}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1052.672904} & \prtime{0.2426} & \prtime{3.21419} & \prtime{1049.1886}& & & &\prtime{ 1871.897413}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.3414}\\
3 & \prtime{8.03342}\\
4 & \prtime{1065.1134}\\
\midrule
 & \prtime{ 1074.510554}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1074.510554} & \prtime{1.3414} & \prtime{8.03342} & \prtime{1065.1134}& & & &\prtime{ 1823.470662}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{9.89065}\\
3 & \prtime{19.7236}\\
4 & \prtime{1094.4166}\\
\midrule
 & \prtime{ 1124.051717}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk32.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1124.051717} & \prtime{9.89065} & \prtime{19.7236} & \prtime{1094.4166}& & & &\prtime{ 1907.609855}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.237459}\\
3 & \prtime{1.20523}\\
4 & \prtime{1069.5139}\\
\midrule
 & \prtime{ 1070.981656}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1070.981656} & \prtime{0.237459} & \prtime{1.20523} & \prtime{1069.5139}& & & &\prtime{ 1716.174741}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.911187}\\
3 & \prtime{4.78787}\\
4 & \prtime{1086.9594}\\
\midrule
 & \prtime{ 1092.679408}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1092.679408} & \prtime{0.911187} & \prtime{4.78787} & \prtime{1086.9594}& & & &\prtime{ 1759.452536}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.31822}\\
3 & \prtime{6.57161}\\
4 & \prtime{1320.3662}\\
\midrule
 & \prtime{ 1328.277890}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1328.277890} & \prtime{1.31822} & \prtime{6.57161} & \prtime{1320.3662}& & & &\prtime{ 1817.450022}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{0.262152}\\
3 & \prtime{1.5288}\\
4 & \prtime{1079.2575}\\
\midrule
 & \prtime{ 1081.073449}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1081.073449} & \prtime{0.262152} & \prtime{1.5288} & \prtime{1079.2575}& & & &\prtime{ 1819.785074}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{1.04566}\\
3 & \prtime{5.1438}\\
4 & \prtime{1080.8235}\\
\midrule
 & \prtime{ 1087.041144}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-2-basis1e-2-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1087.041144} & \prtime{1.04566} & \prtime{5.1438} & \prtime{1080.8235}& & & &\prtime{ 1767.061789}\\


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination.tex <==
\begin{tabular}{rr}
2 & \prtime{4.87825}\\
3 & \prtime{8.15091}\\
4 & \prtime{1414.3094}\\
\midrule
 & \prtime{ 1427.366653}\\
\end{tabular}


==> 181031/sphereii/sphereii10-fmm3logXsub3-dk8.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_elimination2.tex <==
mIFMMb4 & \prtime{ 1427.366653} & \prtime{4.87825} & \prtime{8.15091} & \prtime{1414.3094}& & & &\prtime{ 1832.260147}\\


==> Makefile <==
#TEX = latex # TikZ
TEX = pdflatex # TikZ

#SRC = main.tex
SRC = ms.tex

BIB = paper.bib

XDVI = xdvi
AUX = ${SRC:.tex=.aux}
PDF = ${SRC:.tex=.pdf}
DVI = ${SRC:.tex=.dvi}

yymmdd=$(shell date +%y%m%d_%H%M)

all: ${SRC} ${BIB}
	${TEX} ${SRC}
	bibtex ${AUX}
	${TEX} ${SRC}
#	dvipdfmx ${DVI}
#	${TEX} supplementary.tex #pdflatex does not work
#	dvipdfmx supplementary.dvi
tex: ${SRC}
	${TEX} ${SRC}
xdvi x dvi d:
	${XDVI} ${DVI} &
clean:
	rm -f *.dvi *.log *.aux *.bbl *.blg *.spl core *.out
tar:
	#tar cvfzh ${SRC:.tex=.tgz} Makefile *.tex *.sty *.pdf *.bib 
	tar cvfzh ${SRC:.tex=.tar.gz} Makefile *.tex *.sty *.bib 
pdf:
	dvips ${SRC:.tex=.dvi} # TikZ
	ps2pdf ${SRC:.tex=.ps} # TikZ
b back backup: tar
	mv ${SRC:.tex=.tgz} /home/ttaka/TeX/helm3d/parallel/backup_dropbox/backup/${yymmdd}.tgz
	cp -p ${PDF} /home/ttaka/TeX/helm3d/parallel/backup_dropbox/backup/${yymmdd}.pdf
#tk:
#	pdftk ${PDF} cat 1-34 output ${SRC:.tex=170404.pdf}
#	pdftk ${PDF} cat 35-end output reply170404.pdf
#
#src: 
#	tar cvfz source170404.tgz \
#	pmbb-sym.sty \
#	acknowledgments.tex \
#	conclusion.tex
arxiv:
	tar cvfzh /home/ttaka/tmp/${SRC:.tex=.tgz} Makefile *.tex *.sty *.bbl 181031/*/*.tex 181031/*/*.pgf 181031/*/*.table figure/*.eps figure/*.pdf figure/group/*.eps figure/group/*.pdf elsarticle/*


==> group.tex <==
\iffalse % skip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Intermediate steps to create the groups in Figure \ref{fig:group_example}(a)}\label{s:group_cc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\autoref{fig:cc} illustrates the intermediate steps to divide 38 nodes at level 3 into groups so that any two nodes in every group satisfy the condition in \autoref{eq:sep} where $\separation=3$, as mentioned in \autoref{fig:group_example}(a). In each sub-figure, any two nodes with the thick border (in red) satisfy the condition in \autoref{eq:sep} where $\separation=3$. A node in gray has been already included in a previous group. Finally, we have eight groups, i.e., $G_0$ to $G_7$.



\begin{figure}[h]
  \begin{tabular}{ccc}
    \includegraphics[width=.29\textwidth]{figure/group/fig-cc0}&
    \includegraphics[width=.29\textwidth]{figure/group/fig-cc1}&
    \includegraphics[width=.29\textwidth]{figure/group/fig-cc2}\\
    $G_0$ & $G_1$ & $G_2$\\
    \includegraphics[width=.29\textwidth]{figure/group/fig-cc3}&
    \includegraphics[width=.29\textwidth]{figure/group/fig-cc4}&
    \includegraphics[width=.29\textwidth]{figure/group/fig-cc5}\\
    $G_3$ & $G_4$ & $G_5$\\
    \includegraphics[width=.29\textwidth]{figure/group/fig-cc6}&
    \includegraphics[width=.29\textwidth]{figure/group/fig-cc7}&\\
    % \includegraphics[width=.29\textwidth]{figure/group/fig-cc-group-color}\\
    %$G_6$ & $G_7$ & All the eight groups\\
    $G_6$ & $G_7$ &\\
  \end{tabular}
  \caption{Example of grouping, where 38 nodes are divided to 8 groups, i.e., $G_0$ to $G_7$.}
  \label{fig:cc}
\end{figure}

\fi % skip

\iffalse % skip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Complexity of the grouping algorithm}\label{s:group_complexity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\autoref{fig:group} shows the time to group a given $n$ nodes in a level. The present data was measured in the sphere model (see \autoref{tab:stat_sphereii10}), where the separation parameter $\separation$ was chosen as 3.

\begin{figure}[h]
  \centering
  \def\mydata{}
  \begin{tabular}{cc}
    \includegraphics[width=.5\textwidth]{./181016/sphereii/fig-seek}&
    \includegraphics[width=.5\textwidth]{./181031/office/fig-seek-office05}\\
    Sphere model & Office model
  \end{tabular}
  \caption{Time for grouping in seconds.}
  \label{fig:group}
\end{figure}


  
%ttaka@z sphereii]$ grep seek sphereii10.log-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3 
%# TH00 eliminate_level: level=7: time_elimination_level=7.242339 (seek=0.045444, sort=0.000000)
%# TH00 eliminate_level: level=6: time_elimination_level=27.221092 (seek=0.008410, sort=0.000000)
%# TH00 eliminate_level: level=5: time_elimination_level=7.904348 (seek=0.002212, sort=0.000000)
%# TH00 eliminate_level: level=4: time_elimination_level=2.796887 (seek=0.000641, sort=0.000000)
%# TH00 eliminate_level: level=3: time_elimination_level=1.646342 (seek=0.000198, sort=0.000000)
%# TH00 eliminate_level: level=2: time_elimination_level=3.093193 (seek=0.000284, sort=0.000000)

%[ttaka@z office]$ grep seek office05.log-fmm3logXsep3top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3 
%# TH00 eliminate_level: level=7: time_elimination_level=4.999223 (seek=0.078244, sort=0.000000)
%# TH00 eliminate_level: level=6: time_elimination_level=25.462123 (seek=0.014894, sort=0.000000)
%# TH00 eliminate_level: level=5: time_elimination_level=19.715427 (seek=0.003802, sort=0.000000)
%# TH00 eliminate_level: level=4: time_elimination_level=23.829973 (seek=0.001042, sort=0.000000)
%# TH00 eliminate_level: level=3: time_elimination_level=41.385920 (seek=0.000234, sort=0.000000)
%# TH00 eliminate_level: level=2: time_elimination_level=59.374863 (seek=0.000060, sort=0.000000)


\fi % skip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Proof for sufficient conditions in Eqs.~(\ref{eq:sep3}), (\ref{eq:sep3b}),  and (\ref{eq:sep6})} \label{s:group_proof}
\section{Proofs of no race-condition under the sufficient conditions in Eqs.~(\ref{eq:sep3}), (\ref{eq:sep3b}),  and (\ref{eq:sep6})} \label{s:group_proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Preliminaries}\label{s:group_pre}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%First, we make the following remark on the memory location (address) of operators (see their notations in Remark~\ref{remark:notation} in \autoref{s:fact}):

First, we make the following remarks on the notation and the memory location (address) of operators:
\begin{remark}%[Notation of operator]
  An operator (sub-matrix) $A_{pq}$ stands for an (original or updated) FMM operator between a target node $p$ and source node $q$.
\end{remark}

\begin{remark}%[Notation of memory location]
  The memory location of $A_{pq}$ is denoted by $\&A_{pq}$.
\end{remark}

\begin{remark}%[Memory location of operator]
  %The memory location of $A_{pq}$ is different from that of $A_{p'q'}$ if $p\ne p'$ or $q\ne q'$, where $p$, $p'$, $q$, and $q'$ denote indices of nodes. The memory location of $A_{pq}$ will be denoted by $\&A_{pq}$.
  The memory location of $A_{pq}$ is different from that of $A_{p'q'}$ (i.e., $\& A_{pq}\ne\& A_{p'q'}$) if $p\ne p'$ or $q\ne q'$. If this is the case, we can rewrite the entities of $A_{pq}$ and $A_{p'q'}$ independently and simultaneously.
  \label{remark:memory}
\end{remark}


Second, since the distance in the LHS of \autoref{eq:sep} is based on the maximum norm for 3D vectors, we have the following statement:
\begin{remark}{}
  The triangle inequality $\dist(a,b)\le\dist(a,c)+\dist(c,b)$ holds for any nodes $a$, $b$, and $c$ in the same level.
  \label{remark:tri}
\end{remark}
%Proof: Regarding $\dist(a,b)$, we suppose the $\xi$th component $\abs{\xi_a-\xi_b}$ is larger than the other $\eta$ and $\zeta$th components, where $\xi\in\{x,y,z\}$, $\eta\in\{x,y,z\}\setminus\{\xi\}$, and $\zeta\in\{x,y,z\}\setminus\{\xi,\eta\}$. Then, we have $\dist(a,b)=\abs{\xi_a-\xi_b}\le\abs{\xi_a-\xi_c}+\abs{\xi_c-\xi_b}$ for any node $c$. Here, no matter what values of $\abs{\eta_a-\eta_c}$ and $\abs{\zeta_a-\zeta_c}$ are, it holds that $\abs{\xi_a-\xi_c}\le\max(\abs{\xi_a-\xi_c},\abs{\eta_a-\eta_c},\abs{\zeta_a-\zeta_c})\equiv\dist(a,c)$. Similarly, we have $\abs{\xi_c-\xi_b}\le\dist(c,b)$. The underlying inequality follows from these three inequalities.

Now we will prove the inequalities in Eqs.~(\ref{eq:sep3}), (\ref{eq:sep3b}), and (\ref{eq:sep6}) are sufficient to avoid the data race problems in the cases of (b), (c), and (d), respectively. To this end, we will consider two nodes $i$ and $i'$ in the same level. Then, when we assign threads $T_i$ and $T_{i'}$ to $i$ and $i'$, respectively, we may show that the memory location of the operator where $T_i$ is working does not coincide with that where $T_{i'}$ is working.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof for $\separation\ge 3$ in Eq.~(\ref{eq:sep3})}\label{s:sep3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%No race condition can occur between $T_i$ and $T_{i'}$ whenever they handle different kinds of operator. Therefore, we may consider a certain kind of neighbor-to-neighbor operator, say $X2Y$. Now we let $T_i$ (respectively, $T_{i'}$) handle $X2Y_{pq}$ and $X2Y_{qp}$ (respectively, $X2Y_{p'q'}$ and $X2Y_{q'p'}$), where $p,q\in\NL_i$ (respectively, $p',q'\in\NL_{i'}$). Then, since $\dist(i,i')\ge 3L$ follows from \autoref{eq:sep3}, we have $3L\le\dist(i,i')\le\dist(i,p)+\dist(p,p')+\dist(p',i')$ from Remark~\ref{remark:tri}. Here, $\dist(p,i)\le L$ and $\dist(i',p')\le L$ hold from the definition of the neighbor list. Therefore, we have $\dist(p,p')\ge L$. This means that $p\ne p'$. In the same way, we can show $p\ne q'$, $q\ne p'$, and $q\ne q'$. From Remark~\ref{remark:memory}, we can conclude both $\&X2Y_{pq}$ and $\&X2Y_{qp}$ coincide with neither $\&X2Y_{p'q'}$ nor $\&X2Y_{q'p'}$. Hence, $T_i$ and $T_{i'}$ never fall in a data race condition. $\qedsymbol$

No race condition can occur between $T_i$ and $T_{i'}$ whenever they handle different kinds of operator. Therefore, we may consider a certain kind of neighbor-to-neighbor operator, say $A$. Now we let $T_i$ (respectively, $T_{i'}$) handle $A_{pq}$ and $A_{qp}$ (respectively, $A_{p'q'}$ and $A_{q'p'}$), where $p,q\in\NL_i$ (respectively, $p',q'\in\NL_{i'}$). Then, since $\dist(i,i')\ge 3L$ follows from \autoref{eq:sep3}, we have $3L\le\dist(i,i')\le\dist(i,p)+\dist(p,p')+\dist(p',i')$ from Remark~\ref{remark:tri}. Here, $\dist(p,i)\le L$ and $\dist(i',p')\le L$ hold from the definition of the neighbor list. Therefore, we have $\dist(p,p')\ge L$. This means that $p\ne p'$. In the same way, we can show $p\ne q'$, $q\ne p'$, and $q\ne q'$. From Remark~\ref{remark:memory}, we can conclude both $\&A_{pq}$ and $\&A_{qp}$ coincide with neither $\&A_{p'q'}$ nor $\&A_{q'p'}$. Hence, $T_i$ and $T_{i'}$ never fall in a data race condition. $\qedsymbol$ 
%\todo{I just replaced X2Y with A.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof for $\separation\ge 3$ in Eq.~(\ref{eq:sep3b})}\label{s:sep3b}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In what follows, we consider the child-to-parent operator (i.e., $\MtoM$)
%\todo{Need the adjoint operator? ($\MtoM^*$?)}
but the proof is the same for the parent-to-child operator (i.e., $\LtoL$).

Since $\dist(i,i')\ge 3L$ follows from \autoref{eq:sep3b}, we can write $3L\le\dist(i,i')\le\dist(i,q)+\dist(q,q')+\dist(q',i')$ from Remark~\ref{remark:tri}. Then, from $\dist(q,i)\le L$ and $\dist(i',q')\le L$, we can obtain $3L\le\dist(q,q')+2L~\Rightarrow~\dist(q,q')\ge L~\Rightarrow~q\ne q'$. This means $\&\MtoM_{\tilde{q}q}\ne\&\MtoM_{\tilde{q'}q'}$
%\todo{$\MtoM^*$?}
from Remark~\ref{remark:memory} (even if $\tilde{q}=\tilde{q}'$ holds). $\qedsymbol$


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof for $\separation\ge 6$ in Eq.~(\ref{eq:sep6})}\label{s:sep6}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%We may show that (I)~$\&M2L_{pl}\ne\&M2L_{p'l'}$, (II)~$\&M2L_{pl}\ne\&M2L_{l'p'}$, (III)~$\&M2L_{lp}\ne\&M2L_{p'l'}$, and (IV)~$\&M2L_{lp}\ne\&M2L_{l'p'}$ for any $p\in\NL_i$, $p'\in\NL_{i'}$, $l\in\NL_p\cup\IL_p$, and $l'\in\NL_{p'}\cup\IL_{p'}$\footnote{(I)--(IV) are directly related to the underlined M2L operators regarding $p$ at Lines \ref{line:fact_NY} and \ref{line:fact_NN1} in \autoref{algo:fact}, but the proof for $q$ at Lines~\ref{line:fact_YN} and \ref{line:fact_NN2} is the same.}. From $\separation\ge 6$ in \autoref{eq:sep6} and Remark~\ref{remark:tri}, we have have $6L\le \dist(i,i')\le \dist(i,p)+\dist(p,p')+\dist(p',i')$. Since $\dist(i,p)\le L$ and $\dist(p',i')\le L$ hold, we can obtain $\dist(p,p')\ge 4L~\Rightarrow~p\ne p'$. Then, (I) and (VI) hold from Remark~\ref{remark:memory}. Further, by combining $\dist(p,l)\le 3L$, which holds from the definitions of $\NL_p$ and $\IL_p$, with the aforementioned $\dist(p,p')\ge 4L$, we can obtain $4L\le\dist(p,p')\le\dist(p,l)+\dist(l,p')\le 3L+\dist(l,p')~\Rightarrow~L\le\dist(l,p')~\Rightarrow~l\ne p'$. Then, (II) and (III) hold. $\qedsymbol$ % REMOVDE \NL_p and \NL_{p'}; see the mail from Chao; 190213

%We may show that (I)~$\&M2L_{pl}\ne\&M2L_{p'l'}$, (II)~$\&M2L_{pl}\ne\&M2L_{l'p'}$, (III)~$\&M2L_{lp}\ne\&M2L_{p'l'}$, and (IV)~$\&M2L_{lp}\ne\&M2L_{l'p'}$ for any $p\in\NL_i$, $p'\in\NL_{i'}$, $l\in\IL_p$, and $l'\in\IL_{p'}$\footnote{(I)--(IV) are directly related to the underlined M2L operators regarding $p$ at Lines \ref{line:fact_NY} and \ref{line:fact_NN1} in \autoref{algo:fact}, but the proof for $q$ at Lines~\ref{line:fact_YN} and \ref{line:fact_NN2} is the same.}. From $\separation\ge 6$ in \autoref{eq:sep6} and Remark~\ref{remark:tri}, we have have $6L\le \dist(i,i')\le \dist(i,p)+\dist(p,p')+\dist(p',i')$. Since $\dist(i,p)\le L$ and $\dist(p',i')\le L$ hold, we can obtain $\dist(p,p')\ge 4L~\Rightarrow~p\ne p'$. Then, (I) and (VI) hold from Remark~\ref{remark:memory}. Further, by combining $\dist(p,l)\le 3L$, which holds from the definition of $\IL_p$, with the aforementioned $\dist(p,p')\ge 4L$, we can obtain $4L\le\dist(p,p')\le\dist(p,l)+\dist(l,p')\le 3L+\dist(l,p')~\Rightarrow~L\le\dist(l,p')~\Rightarrow~l\ne p'$. Then, (II) and (III) hold. $\qedsymbol$ % REMOVDE \NL_p and \NL_{p'}; see the mail from Chao; 190213

We may show that (I)~$\&\MtoL_{pl}\ne\&\MtoL_{p'l'}$, (II)~$\&\MtoL_{pl}\ne\&\MtoL_{l'p'}$, (III)~$\&\MtoL_{lp}\ne\&\MtoL_{p'l'}$, and (IV)~$\&\MtoL_{lp}\ne\&\MtoL_{l'p'}$ for any $p\in\NL_i$, $p'\in\NL_{i'}$, $l\in\IL_p$, and $l'\in\IL_{p'}$\footnote{(I)--(IV) are directly related to the underlined $\MtoL$ operators regarding $p$ at Line \ref{line:fact_NN1} in \autoref{algo:fact}, but the proof for $q$ at Lines~\ref{line:fact_YN} and \ref{line:fact_NN2} is the same.}. From $\separation\ge 6$ in \autoref{eq:sep6} and Remark~\ref{remark:tri}, we have have $6L\le \dist(i,i')\le \dist(i,p)+\dist(p,p')+\dist(p',i')$. Since $\dist(i,p)\le L$ and $\dist(p',i')\le L$ hold, we can obtain $\dist(p,p')\ge 4L~\Rightarrow~p\ne p'$. Then, (I) and (VI) hold from Remark~\ref{remark:memory}. Further, by combining $\dist(p,l)\le 3L$, which holds from the definition of $\IL_p$, with the aforementioned $\dist(p,p')\ge 4L$, we can obtain $4L\le\dist(p,p')\le\dist(p,l)+\dist(l,p')\le 3L+\dist(l,p')~\Rightarrow~L\le\dist(l,p')~\Rightarrow~l\ne p'$. Then, (II) and (III) hold. $\qedsymbol$ % REMOVDE \NL_p and \NL_{p'}; see the mail from Chao; 190213
%\todo{I just replaced M2L with K.}

%\iffalse
%
%As a reference, \autoref{fig:sep6} illustrates a specific case that $i$ and $i'$ are separated by $6L$ in $x$-direction.
%
%\begin{figure}[htb]
%  \centering
%  \includegraphics[width=.7\textwidth]{figure/fig-sep6-1D}
%  \caption{Example of two nodes $i$ and $i'$ separated by $6L$ in $x$-direction. Here, $p\in\NL_i$, $p'\in\NL_{i'}$, $l\in\NL_i\cup\IL_i$, and thick lines denote the partitions of parent nodes. Clearly, $i\ne i'$ holds. In addition, this figure illustrates that $\dist(l,p')\ge L$ (thus, $l\ne p'$) and $\dist(p,p')\ge 4L$ (thus, $p\ne p'$). Note that we may consider an alternative layout of the partitions at the parent level, i.e., all the portions are shifted by one in $x$-direction. In this case, we can say $\dist(l,p')\ge 2L$ (thus, $l\ne p'$) instead of $\dist(l,p')\ge L$. Therefore, we can prove the statement similarly.}
%  \label{fig:sep6}
%\end{figure}
%
%\fi


==> office_profile.tex <==
%\section{Details for the office model}\label{s:office_profile}
\section{Survey of the best settings for the Office model (Section~\ref{s:office}}\label{s:office_profile}

%We examined the best settings of BD, mIFMM, and nIFMM regarding the office model in Section~\ref{s:office} of the main article.


%\subsection{Survey of the best BD}\label{s:office_BD}
\subsection{BD}\label{s:office_BD}

We first determined the best value of $\lBD$ for BD. From the result in Table~\ref{tab:office05_BD} and Figure~\ref{fig:office05_BD_total}, \textbf{BDbot4} was nearly the best for $k\le 32$ and \textbf{BDbot3} for $k=64$. For the sake of fair comparison with nIFMM as well as mIFMM, we choose the best result (that is, shortest computation time) of BD for every wavenumber when we draw Figure~\ref{fig:office05_speedup} of the main article. 

We note that BDbot2 required too much memory (for precomputing the block diagonals) to run. In addition, we could not perform BDbot5, 6, and 7 in the case of $k=64$ because of the limitation of computation time, i.e., 24 hours.


\begin{table}[h]
  \centering
  \caption{Profile of \textbf{BD} for the \textbf{office} model. The speedup (``\tsp'') as well as the discrepancy (``\disc'') is relative to BDbot3, which is the best BD for $k=64$.}
    %Note that we could not run BDbot2 because of the out of memory for any $k$ and BDbot5, 6, and 7 for $k=64$ within the time limitation of 24 hours.}
    % See Section~\ref{s:office_comp3}.}
  \label{tab:office05_BD}
  % 
  \def\mydata{./181031/office}
  % \def\llerr{\disc}
  \def\merr{\disc}
  % 
  \scriptsize
  %\small
  \myinputII{\mydata/office05-fmm3logBDX0-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0.tex}{}{}{}{}{}{}{}{1}
  \myinputII{\mydata/office05-fmm3logBDX1-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logBDX2-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logBDX3-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logBDX4-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logBDX5-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0.tex}{}{}{}{}{}{}{}{2}
\end{table}



\begin{figure}[h]
  \centering
  \def\mydata{./181031/office}
  
  \begin{tikzpicture}%[scale=0.9, every node/.style={scale=0.9}]
    \begin{axis}[
      % title={$\varepsilon=10^{-3}$},
      xlabel={Wavenumber $k$},
      ylabel style={align=center},
      ylabel={Total computation time [sec]},
      xmode=log,
      ymode=log,
      xmin=1, xmax=100,
      % ymin=0.0, ymax=3.0, ytick={0.0,0.5,...,3.0},
      ymin=100, ymax=100000,
      legend pos=south east,
      legend cell align={left},
      ymajorgrids=true,
      grid style=dashed,
      legend entries={BDb7, BDb6, BDb5, BDb4, BDb3},
      ]
      
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logBDX0-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logBDX1-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logBDX2-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logBDX3-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logBDX4-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc0_total.pgf};
      
    \end{axis}
  \end{tikzpicture}
  \caption{Total computation time of \textbf{BD} for the \textbf{office} model.} %BDb3 is not shown because its computation time was very large.
  \label{fig:office05_BD_total}
\end{figure}


%\subsection{Survey of the best mIFMM}\label{s:office_mIFMM}
\subsection{mIFMM}\label{s:office_mIFMM}

As seen in Figure~\ref{fig:office05_mIFMM_total}, the best mIFMM was \textbf{mIFMMbot5} (i.e., $\ell=5$) when we varied $\ell$ from 7 to 4. Although the number of iterations (``\niter'') is relatively small for every wavenumber, the performance of $\ell=4$ was clearly worse than that of $\ell=5$; see Table~\ref{tab:office05_mIFMM}.



Note that $k=64$ of $\ell=7$ did not run due to the out of memory.


%\todo{mIFMMb7 1e-3; tmp18.sh; 11/26 0pm}
%\todo{mIFMMb6 1e-3; tmp6.sh}
%\todo{mIFMMb5 1e-3; tmp19.sh; 11/26 0pm}
%\todo{mIFMMb4 1e-3; tmp26.sh; 11/27 9am}

\begin{table}[h]
  \centering
  \caption{Profile of \textbf{mIFMM} for the \textbf{office} model. The speedup (``\tsp'') as well as the discrepancy (``\disc'') is relative to BDbot3, which is the best BD for $k=64$.}
    %The numbers in the column of ``Precon.'' denote the values of $\varepsilon$.
    %Note that we could not run mIFMMbot7 for $k=64$ because of the out of memory. See Section~\ref{s:office_comp3}.}
  \label{tab:office05_mIFMM}
  % 
  %\def\mydata{./181016/office}
  \def\mydata{./181031/office}
  %\def\llerr{\disc}
  \def\merr{\disc}
  % 
  \scriptsize
  %\small
  \myinputII{\mydata/office05-fmm3logXsub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{1}
  \myinputII{\mydata/office05-fmm3logXsub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logXsub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logXsub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{2}
\end{table}


\begin{figure}[h]
  \centering
  \def\mydata{./181031/office}
  
  \begin{tikzpicture}%[scale=0.9, every node/.style={scale=0.9}]
    \begin{axis}[
      % title={$\varepsilon=10^{-3}$},
      xlabel={Wavenumber $k$},
      ylabel style={align=center},
      ylabel={Total computation time [sec]},
      xmode=log,
      ymode=log,
      xmin=1, xmax=100,
      % ymin=0.0, ymax=3.0, ytick={0.0,0.5,...,3.0},
      ymin=1000, ymax=100000,
      legend pos=north west,
      legend cell align={left},
      ymajorgrids=true,
      grid style=dashed,
      legend entries={mIFMMb7, mIFMMb6, mIFMMb5, mIFMMb4}
      ]
      
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logXsub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logXsub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logXsub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logXsub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_total.pgf};
      
    \end{axis}
  \end{tikzpicture}
  \caption{Total computation time of \textbf{mIFMM} for the \textbf{office} model.}
  \label{fig:office05_mIFMM_total}
\end{figure}

%\subsection{Survey of the best nIFMM}\label{s:office_nIFMM}
\subsection{nIFMM}\label{s:office_nIFMM}

We tested nIFMM with varying the top level $\tau$ from 2 to 3 and the bottom level $\ell$ from 7 to 4. Basically, $\tau=3$ gave better results than $\tau=2$. Therefore, we show only the result of $\tau=3$ in Table~\ref{tab:office05_nIFMM} From Figure~\ref{fig:office05_nIFMM_total}, we determined \textbf{nIFMMsep3top3bot5} as the best.


The tendency of both initialization (``\init'') and factorization times  (``\elim'') as well as the number of iterations (``\niter'') are similar to that of mIFMM in Table
~\ref{tab:office05_mIFMM}. However, the preconditioning (``\ms'') and factorization were accelerated by the node-based parallelization. 


Note that $k=64$ of $\ell=7$ did not run due to the out of memory.

%\todo{nIFMMs3t2b7 1e-3; tmp23.sh; 11/26 10pm}
%\todo{nIFMMs3t2b6 1e-3; tmp14.sh; 11/26 9am}
%\todo{nIFMMs3t2b5 1e-3; tmp24.sh; 11/26 10pm}
%\todo{nIFMMs3t2b4 1e-3; tmp22.sh; 11/26 10pm}
%\todo{nIFMMs3t3b7 1e-3; tmp25.sh; 11/26 10pm}
%\todo{nIFMMs3t3b6 1e-3; tmp1.sh}
%\todo{nIFMMs3t3b5 1e-3; tmp20.sh; 11/26 10pm}
%\todo{nIFMMs3t3b4 1e-3; tmp21.sh; 11/26 10pm}

\begin{table}[h]
  \centering
  \caption{Profile of \textbf{nIFMM} for the \textbf{office} model. The speedup (``\tsp'') as well as the discrepancy (``\disc'') is relative to BDbot3, which is the best BD for $k=64$.}
  % The numbers in the column of ``Precon.'' denote the values of $\varepsilon$.
  % Note that we could not run nIFMMsep3top3bot7 for $k=64$ because of the out of memory. See Section~\ref{s:office_comp3}.}
  \label{tab:office05_nIFMM}
  % 
  % \def\mydata{./181016/office}
  \def\mydata{./181031/office}
  % \def\llerr{\disc}
  \def\merr{\disc}
  % 
  \scriptsize
  % \small
  \iffalse % SKIP
  $\separation=3$, $\tau=2$\\
  \myinputII{\mydata/office05-fmm3logXsep3top2sub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{1}
  \myinputII{\mydata/office05-fmm3logXsep3top2sub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logXsep3top2sub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logXsep3top2sub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{2}
  $\separation=3$, $\tau=3$\\
  \fi % SKIP
  \myinputII{\mydata/office05-fmm3logXsep3top3sub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{1}
  \myinputII{\mydata/office05-fmm3logXsep3top3sub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logXsep3top3sub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/office05-fmm3logXsep3top3sub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{2}
\end{table}



\begin{figure}[h]
  \centering
  \def\mydata{./181031/office}
  
  \begin{tikzpicture}%[scale=0.9, every node/.style={scale=0.9}]
    \begin{axis}[
      % title={$\varepsilon=10^{-3}$},
      xlabel={Wavenumber $k$},
      ylabel style={align=center},
      ylabel={Total computation time [sec]},
      xmode=log,
      ymode=log,
      xmin=1, xmax=100,
      % ymin=0.0, ymax=3.0, ytick={0.0,0.5,...,3.0},
      ymin=100, ymax=10000,
      legend pos=south east,
      legend cell align={left},
      ymajorgrids=true,
      grid style=dashed,
      legend entries={nIFMMs3t3b7, nIFMMs3t3b6, nIFMMs3t3b5, nIFMMs3t3b4}
      ]
      
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logXsep3top3sub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logXsep3top3sub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logXsep3top3sub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/office05-fmm3logXsep3top3sub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc0-fillin1e-3-basis1e-3-LR3_total.pgf};
      
    \end{axis}
  \end{tikzpicture}
  \caption{Total computation time of \textbf{nIFMM} for the \textbf{office} model.}  %The results of $\tau=2$ and 4 are omitted.} %mIFMMb4 is not shown because its computation time was very large.
  \label{fig:office05_nIFMM_total}
\end{figure}


%
%\begin{figure}[h]
%  \centering
%  % \def\mydata{./180629/office}
%  %\def\mydata{./180718/office}
%  \def\mydata{./181031/office}
%  % 
%  \begin{tabular}{cc}
%    \includegraphics[width=.4\textwidth]{\mydata/fig-time-total-office05-delta7-epsilon1e-3}
%    &\includegraphics[width=.4\textwidth]{\mydata/fig-niter-office05-delta7-epsilon1e-3}\\
%    \includegraphics[width=.4\textwidth]{\mydata/fig-tsp-office05-delta7-epsilon1e-3}
%    &\includegraphics[width=.4\textwidth]{\mydata/fig-speedup-office05-delta7-epsilon1e-3}
%  \end{tabular}
%  % 
%  \caption{Performance of nIFMMsep3top3bot6, mIFMMbot6, and BDbot4 in the \textbf{office} model in the case of $\varepsilon=10^{-3}$. (Top left) Total computation time. (Top right) Number of iterations. (Bottom left) Speedup of the nIFMM and the mIFMM relative to the BD. (Bottom right) Speedup of the nIFMM relative to the mIFMM. See Section~\ref{s:office}.}
%  \label{fig:office05}
%\end{figure}


==> sphere_profile.tex <==
%\section{Details for sphere model}\label{s:sphereii_details}
%\section{Sphere model}\label{s:sphereii_details}
\section{Survey of the best settings for the Sphere model (Section~\ref{s:sphere})}\label{s:sphereii_details}


%In Section~\ref{s:sphere} of the main article, we mentioned that \textbf{BDbot5}, \textbf{mIFMMbot6}, and \textbf{nIFMMsep3top3bot6} are the best. The reason is given below, with using the performance profiles of the three preconditioners.


%\subsection{Survey of the best BD}\label{s:sphereii_BD}
\subsection{BD}\label{s:sphereii_BD}


To make a fair comparison with the IFMM-based preconditioners, we investigated the best value of the bottom level $\lBD$. The timing results of the FMBEM based on the BD using $\lBD$ of $3$ to $7$ are compared in Table~\ref{tab:sphereii10_BD}. As $\lBD$ decreased, the number of iterations (in the column ``\niter'') basically decreased but both initialization (``\init'') and preconditioning times (``\ms'') increased. As a result, $\lBD=5$ was the best in terms of the total computation time, as seen in Figure~\ref{fig:sphereii10_BD_total}.  We thus determined \textbf{BDbot5} as the best BD.


\begin{table}[h]
  \centering
  \caption{Profile of \textbf{BD} for the \textbf{sphere} model. The speedup (``\tsp'') is relative to BDbot5. See Section~\ref{s:sphereii_BD}.}
  \label{tab:sphereii10_BD}
  % 
  %\def\mydata{./181016/sphereii}
  \def\mydata{./181031/sphereii}
  % 
  \scriptsize
  \myinputII{\mydata/sphereii10-fmm3logBDX0-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95.tex}{}{}{}{}{}{}{}{1}
  \myinputII{\mydata/sphereii10-fmm3logBDX1-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/sphereii10-fmm3logBDX2-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/sphereii10-fmm3logBDX3-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/sphereii10-fmm3logBDX4-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95.tex}{}{}{}{}{}{}{}{2}
\end{table}


\begin{figure}[h]
  \centering
  \def\mydata{./181031/sphereii}
  

  \begin{tikzpicture}%[scale=0.9, every node/.style={scale=0.9}]
    \begin{axis}[
        %colorbrewer cycle list=Dark2, % INCORRECT
        %cycle list/Set1, % WORKS BUT NO MARKS
        % title={$\varepsilon=10^{-3}$},
        xlabel={Wavenumber $k$},
        ylabel style={align=center},
        ylabel={Total computation time [sec]},
        xmode=log,
        ymode=log,
        xmin=1, xmax=100,
        % ymin=0.0, ymax=3.0, ytick={0.0,0.5,...,3.0},
        ymin=100, ymax=10000,
        %legend pos=south east,
        legend pos=north west,
        legend cell align={left},
        ymajorgrids=true,
        grid style=dashed,
        legend entries={BDb7, BDb6, BDb5, BDb4, BDb3},
      ]

      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logBDX0-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logBDX1-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logBDX2-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logBDX3-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logBDX4-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95_total.pgf};
      
    \end{axis}
  \end{tikzpicture}
  \caption{Total computation time of \textbf{BD} for the \textbf{sphere} model.} %BDb3 is not shown because its computation time was very large.
  \label{fig:sphereii10_BD_total}
\end{figure}



\iffalse % SUPPLEMENTARY
\input{tab_legend}
\fi


%\subsection{Survey of the best mIFMM}\label{s:sphereii_mIFMM}
\subsection{mIFMM}\label{s:sphereii_mIFMM}


We measured the performance of mIFMM with varying its depth $\ell$ from $4$ to $7$ ($=\lFMM$). Table~\ref{tab:sphereii10_mIFMM} shows the result. In comparison with BD in Table~\ref{tab:sphereii10_BD}, the number of iterations (in the column ``\niter'') decreased significantly. We can observe that, although the highest speedup relative to the best BD (``\tsp'') was only $1.1$ at $k=32$, $\ell=6$ is the fastest (Figure~\ref{fig:sphereii10_mIFMM_total}). We thus determined \textbf{mIFMMbot5} as the best.

We note that mIFMM could not run $k=32$ with $\ell=7$ because the out of memory occurred during the initialization for level $7$.


\begin{table}[h]
  \centering
  \caption{Profile of \textbf{mIFMM} for the \textbf{sphere} model. The speedup (``\tsp'') is relative to the best BD (i.e., BDbot5).} %See Section~\ref{s:sphereii_mIFMM}.}
  \label{tab:sphereii10_mIFMM}
  % 
  %\def\mydata{./181016/sphereii}
  \def\mydata{./181031/sphereii}
  % 
  \scriptsize
  %
  \myinputII{\mydata/sphereii10-fmm3logXsub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{1}
  \myinputII{\mydata/sphereii10-fmm3logXsub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/sphereii10-fmm3logXsub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/sphereii10-fmm3logXsub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{2}
\end{table}


\begin{figure}[]
  \centering
  \def\mydata{./181031/sphereii}
  
  \begin{tikzpicture}%[scale=0.9, every node/.style={scale=0.9}]
    \begin{axis}[
      % title={$\varepsilon=10^{-3}$},
      xlabel={Wavenumber $k$},
      ylabel style={align=center},
      ylabel={Total computation time [sec]},
      xmode=log,
      ymode=log,
      xmin=1, xmax=100,
      % ymin=0.0, ymax=3.0, ytick={0.0,0.5,...,3.0},
      ymin=100, ymax=100000,
      legend pos=north west,
      legend cell align={left},
      ymajorgrids=true,
      grid style=dashed,
      legend entries={mIFMMb7, mIFMMb6, mIFMMb5, mIFMMb4}
      ]
      
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logXsub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logXsub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logXsub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logXsub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_total.pgf};
      
      
    \end{axis}
  \end{tikzpicture}
  \caption{Total computation time of \textbf{mIFMM} for the \textbf{sphere} model.} %mIFMMb4 is not shown because its computation time was very large.
  \label{fig:sphereii10_mIFMM_total}
\end{figure}


%\subsection{Survey of the best nIFMM}\label{s:sphereii_nIFMM}
\subsection{nIFMM}\label{s:sphereii_nIFMM}


We explored the best setting of nIFMM, with varying $\tau$ from $2$ to $4$ and $\ell$ from $4$ to $7$ and fixing $\separation$ to $3$. Table~\ref{tab:sphereii10_nIFMM} clearly shows that nIFMM reduces its total computation time (``\main'') by reducing the number of iterations (``\niter'') at the cost of the preconditioning (``\ms''), initialization (``\init''), and factorization (``\elim''). As a result, \textbf{nIFMMsep3top3bot6} was determined as the best from Figure~\ref{fig:sphereii10_nIFMM_total}, where only the result of $\tau=3$ is shown because the remaining $\tau=2$ and $4$ were slightly worse than $\tau=3$ in terms of the total computation time. 

Since the initialization routine is common to all the IFMM-based preconditioners, similaly to mIFMM, nIFMM could not perform $k=32$ with $\ell=7$ because the out of memory in the initialization of level $7$.

\begin{table}[h]
  \centering
  \caption{Profile of \textbf{nIFMM} for the \textbf{sphere} model. The speedup (``\tsp'') is relative to the best BD (i.e., BDbot5).} %See Section~\ref{s:sphereii_nIFMM}.}
  \label{tab:sphereii10_nIFMM}
  % 
  % \def\mydata{./181016/sphereii}
  \def\mydata{./181031/sphereii}
  % 
  \scriptsize
  % \myinputII{\mydata/sphereii10-fmm3logBDX2-ngauss4-jpre3-tol1e-5-maxepc040-delta7-inc95.tex}{}{}{}{}{}{}{}{1}
  % 
  % $\separation=3$, $\tau=2$\\
  % \myinputII{\mydata/sphereii10-fmm3logXsep3top2sub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{1}
  % \myinputII{\mydata/sphereii10-fmm3logXsep3top2sub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  % \myinputII{\mydata/sphereii10-fmm3logXsep3top2sub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  % \myinputII{\mydata/sphereii10-fmm3logXsep3top2sub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{2}
  % 
  % $\separation=3$, $\tau=3$\\
  \myinputII{\mydata/sphereii10-fmm3logXsep3top3sub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{1}
  \myinputII{\mydata/sphereii10-fmm3logXsep3top3sub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/sphereii10-fmm3logXsep3top3sub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  \myinputII{\mydata/sphereii10-fmm3logXsep3top3sub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{2}
  % 
  % $\separation=3$, $\tau=4$\\
  % \myinputII{\mydata/sphereii10-fmm3logXsep3top4sub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  % \myinputII{\mydata/sphereii10-fmm3logXsep3top4sub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  % \myinputII{\mydata/sphereii10-fmm3logXsep3top4sub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{0}
  % \myinputII{\mydata/sphereii10-fmm3logXsep3top4sub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3.tex}{}{}{}{}{}{}{}{2}
\end{table}


\begin{figure}[h]
  \centering
  \def\mydata{./181031/sphereii}
  
  \begin{tikzpicture}%[scale=0.9, every node/.style={scale=0.9}]
    \begin{axis}[
      % title={$\varepsilon=10^{-3}$},
      xlabel={Wavenumber $k$},
      ylabel style={align=center},
      ylabel={Total computation time [sec]},
      xmode=log,
      ymode=log,
      xmin=1, xmax=100,
      % ymin=0.0, ymax=3.0, ytick={0.0,0.5,...,3.0},
      ymin=100, ymax=100000,
      legend pos=north west,
      legend cell align={left},
      ymajorgrids=true,
      grid style=dashed,
      legend entries={nIFMMs3t3b7, nIFMMs3t3b6, nIFMMs3t3b5, nIFMMs3t3b4}
      ]
      
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logXsep3top3sub0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logXsep3top3sub1-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logXsep3top3sub2-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_total.pgf};
      \addplot table [x=k, y=total] {\mydata/sphereii10-fmm3logXsep3top3sub3-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-1-basis1e-1-LR3_total.pgf};
      
      
    \end{axis}
  \end{tikzpicture}
  \caption{Total computation time of \textbf{nIFMM} for the \textbf{sphere} model.} %The results of $\tau=2$ and 4 are omitted.} %mIFMMb4 is not shown because its computation time was very large.
  \label{fig:sphereii10_nIFMM_total}
\end{figure}


==> tab_legend.tex <==
\begin{table}[h]
%  \caption{Headings commonly used for Tables \ref{tab:sphereii10_BD}, \ref{tab:sphereii10_mIFMM}, \ref{tab:sphereii10_nIFMM} \ref{tab:sphereii10_low}, \ref{tab:office05_BD}, \ref{tab:office05_mIFMM}, and \ref{tab:office05_nIFMM}.}
\iffalse % SUPPLEMENTARY
  \caption{Headings commonly used for Tables~\ref{tab:sphereii10_BD}, \ref{tab:sphereii10_mIFMM}, \ref{tab:sphereii10_nIFMM}, \ref{tab:office05_BD}, \ref{tab:office05_mIFMM}, and \ref{tab:office05_nIFMM}.}
\else
  \caption{Headings commonly used for Tables~\ref{tab:sphereii10_BD}--\ref{tab:office05_nIFMM}.}
\fi
  \label{tab:legend}
  % 
  %\begin{tabular}{|c|p{.8\textwidth}|}
  \begin{tabular}{|p{.15\textwidth}|p{.8\textwidth}|}
    \toprule
    Legend & Meaning\\
    \midrule
    %\textbf{Precon.} & Preconditioner: \textbf{BD} (block-diagonal), \textbf{nIFMM} (node-based parallel IFMM), or \textbf{mIFMM} (matrix-based parallel IFMM). The numbers (such as ``1e-3'') denote the values of the IFMM's precision parameter $\varepsilon$.\\
    \textbf{Precon.} & Preconditioner of \textbf{BD}, \textbf{nIFMM}, or \textbf{mIFMM}. The numbers (such as ``1e-3'') denote the values of the IFMM's precision parameter $\varepsilon$.\\
    \midrule
    \textbf{$k$} & Wavenumber.\\
    \midrule
    %\textbf{\niter} & Number of GMRES iterations until convergence for a given tolerance ``$tol$''.\\
    \textbf{\niter} & Number of GMRES iterations until convergence.\\
    % \midrule
    % \textbf{\nsp} & Speedup relative to the BD preconditioner in terms of the number of iterations.\\
    \midrule
    %\textbf{\main} & Total computation time (in seconds), which includes everything from the start to the end of an analysis. This is decomposed into the following dominant components: \textbf{\ptop}, \textbf{\gmres}, \textbf{\mv}, \textbf{\ms}, \textbf{\init} and \textbf{\elim}. Recall \autoref{algo:fmbem}.\\
    %\textbf{\main} & Total computation time (in seconds). This is decomposed into the dominant components: \textbf{\ptop}, \textbf{\gmres}, \textbf{\mv}, \textbf{\ms}, \textbf{\init}, and \textbf{\elim}. See \autoref{algo:fmbem}.\\
    \textbf{\main} & Total computation time (in seconds) to perform the FMBEM. This is decomposed into the dominant components: \textbf{\ptop}, \textbf{\gmres}, \textbf{\mv}, \textbf{\ms}, \textbf{\init}, and \textbf{\elim}.\\
    \midrule
    \textbf{\tsp} & Speedup in terms of the total computation time.\\
    \midrule
    \textbf{\ptop} & Time to precompute the P2P operators for FMM.\\%, which are partially reused for IFMM.\\
    \midrule
    %\textbf{\gmres} & Time spent performing GMRES except for its auxiliary routines, i.e., the following preconditioning and matrix-vector product. In our implementation, we cannot measure \textbf{\gmres} directly and, thus, estimate it from the time spent for the entire of GMRES, \textbf{\mv}, and \textbf{\ms}. Then, the estimated time can be \uline{negative} due to the lack of the exact timing measurement, especially, when the number of iterations is small.\\ %because of the timing measurement error$^\dagger$.\\
    %\textbf{\gmres} & Time spent performing GMRES except for the times spent for the following preconditioning and matrix-vector product. Since our implementation cannot measure \textbf{\gmres} directly, we estimate it from the entire time of GMRES, \textbf{\mv}, and \textbf{\ms}. Then, \textbf{\gmres} can be \uline{negative} due to the lack of the exact timing measurement, especially, when \textbf{niter} is small.\\ %because of the timing measurement error$^\dagger$.\\
    \textbf{\gmres} & Time to perform GMRES except for the following preconditioning and matrix-vector product routines. We estimate \textbf{\gmres} from the entire time of GMRES, \textbf{\mv}, and \textbf{\ms}. As a result, \textbf{\gmres} can be \uline{negative} due to the lack of the exact timing measurement, especially, when \textbf{niter} is small.\\
    \midrule
    %\textbf{\mv} & Time spent performing matrix-vector products with the LFFMM. The number of products performed during an analysis is $\textbf{\niter}+1$; the extra one is for performing the RHS vector $b$ of the system equations $Ax=b$.\\
    \textbf{\mv} & Time to perform matrix-vector products with the LFFMM. The number of products results in $\textbf{\niter}+1$; the extra one is to compute the RHS vector $b$.\\
    \midrule
    %\textbf{\ms} & Time to apply the preconditioner in GMRES. The application is repeated $\textbf{niter}+2$ times until convergence if no restart occurs.\\
    \textbf{\ms} & Time to apply the preconditioner in GMRES. The number of applications results in $\textbf{niter}+2$.\\
    \midrule
    %\textbf{\init} & Time spent for the initialization. In the case of the IFMM-based preconditioners, \textbf{\init} corresponds to the time for the initialization phase (see \autoref{s:overview}). In the case of BD, \textbf{\init} corresponds to the time to compute the block diagonals of the preconditioner $M$ and factorize the diagonals (see \autoref{s:precon_bd})\\
    \textbf{\init} & Time to initialize (precompute) the preconditioing. See the details in Lines \ref{line:init_start}--\ref{line:init_end} of Algorithm~\ref{algo:fmbem}. \\
    \midrule
    \textbf{\elim} & Time to perform the factorization phase in the IFMM-based preconditioners.\\
    \midrule
    \iffalse % l2
    %\iftrue % l2
    %\textbf{\llerr} & $l_2$-error of the numerical solution relative to the exact solution in terms of the wave field $u$, i.e., $\mathbf{\llerr}:=\frac{\norm{u_{\rm target}-u_{\rm exact}}_2}{\norm{u_{\rm exact}}_2}$, where $u_{\rm target}\in\bbbc^N$ denotes the numerical solution computed with a target preconditioner (i.e., nIFMM, mIFMM, BD) and $u_{\rm exact}\in\bbbc^N$ denotes the corresponding exact solution of the sphere model.\\
    \textbf{\llerr} & relative $l_2$-error of the wave field $u$, i.e., $\textbf{\llerr}:=\frac{\norm{u_{\rm target}-u_{\rm exact}}_2}{\norm{u_{\rm exact}}_2}$, where $u_{\rm target}\in\bbbc^N$ denotes the numerical solution computed with a target preconditioner (i.e., nIFMM, mIFMM, BD) and $u_{\rm exact}\in\bbbc^N$ denotes the corresponding exact solution. This is only for the sphere model.\\
    \else % linf
    %\textbf{\merr} & $l_\infty$-error of the numerical solution relative to the exact solution in terms of the wave field $u$, i.e., $\mathbf{\merr}:=\frac{\norm{u_{\rm target}-u_{\rm exact}}_\infty}{\norm{u_{\rm exact}}_\infty}$, where $u_{\rm target}\in\bbbc^N$ denotes the numerical solution computed with a target preconditioner (i.e., nIFMM, mIFMM, BD) and $u_{\rm exact}\in\bbbc^N$ denotes the corresponding exact solution of the sphere model.\\
    \textbf{\merr}\quad(sphere model only) & Relative $l_\infty$-error of the wave field $u$, i.e., $\textbf{\merr}:=\frac{\norm{u_{\rm target}-u_{\rm exact}}_\infty}{\norm{u_{\rm exact}}_\infty}$, where $u_{\rm target}\in\bbbc^N$ is the solution computed with a target preconditioner (i.e., nIFMM, mIFMM, BD) and $u_{\rm exact}\in\bbbc^N$ is the corresponding exact solution.\\
    %This is only for the sphere model.\\
    \fi
    \midrule
    \iffalse % l2
    \textbf{\disc} & Relative discrepancy of the solution $u_{\rm IFMM}\in\bbbc^N$ computed with nIFMM or mIFMM from the reference solution $u_{\rm BD}\in\bbbc^N$ computed with BD, i.e., $\textbf{\disc}:=\frac{\norm{u_{\rm IFMM}-u_{\rm BD}}_2}{\norm{u_{\rm BD}}_2}$. This is used to measure the relative accuracy of nIFMM and mIFMM in the office model, for which the exact solution is unavailable.\\
    \else
    \textbf{\disc}\quad\quad\quad\quad(office model only) & Relative discrepancy of the solution $u_{\rm IFMM}\in\bbbc^N$ computed with nIFMM or mIFMM from the reference solution $u_{\rm BD}\in\bbbc^N$ computed with BD, i.e., $\textbf{\disc}:=\frac{\norm{u_{\rm IFMM}-u_{\rm BD}}_\infty}{\norm{u_{\rm BD}}_\infty}$.\\
    %This is used to measure the relative accuracy of nIFMM and mIFMM in the office model, for which the exact solution is unavailable.\\
    \fi
    \bottomrule
  \end{tabular}\\
  %${}^\dagger$ We directly measured $\textbf{\niter}$, $\textbf{\mv}$ ($=:t_1$), $\textbf{\ms}$ ($=:t_2$), and $\textbf{\gmres}+\textbf{\mv}\times\frac{\textbf{\niter}}{\textbf{\niter}+1}+\textbf{\ms}$ ($=:t_3$). Then, we calculated $\textbf{\gmres}$ as $t_3-t_1\frac{\textbf{\niter}}{\textbf{\niter}+1}-t_2$.
\end{table}


==> tab_stat_sphere_sigma6.tex <==
%[ttaka@z sphereii]$ pwd
% /home/ttaka/study/helm3d/181031/g/sphereii
%[ttaka@z sphereii]$ less sphereii10.log-fmm3logXsep6top2sub0-dk4.0-ngauss4-jpre10-tol1e-5-maxepc040-delta7-inc95-fillin1e-3-basis1e-3-LR3_FMM_tree: level= 4: nnodes=1160 (28.3) nleaves=0 ( 0.0) ave_pnt=0.000000 ave_ngbr=14.4 ave_Ilist=46.6
%# TH00 statistics_concurrent_nodes: level=2 nnodes=56 sum=56 ave=1.000000 min=1 max=1 nelim=56.000000 sp=1.000000
%# TH00 statistics_concurrent_nodes: level=3 nnodes=272 sum=112 ave=2.428571 min=2 max=3 nelim=112.000000 sp=2.428571
%# TH00 statistics_concurrent_nodes: level=4 nnodes=1160 sum=142 ave=8.169014 min=4 max=15 nelim=142.000000 sp=8.169014
%# TH00 statistics_concurrent_nodes: level=5 nnodes=4742 sum=181 ave=26.198895 min=5 max=52 nelim=384.000000 sp=12.348958
%# TH00 statistics_concurrent_nodes: level=6 nnodes=18488 sum=208 ave=88.884615 min=6 max=205 nelim=1254.000000 sp=14.743222
%# TH00 statistics_concurrent_nodes: level=7 nnodes=70896 sum=216 ave=328.222222 min=8 max=802 nelim=4531.000000 sp=15.646877

\begin{table}[h]
  \def\prave#1{{\nprounddigits{0}\numprint{#1}}}
  \centering
  \caption{Statistics of nIFMM using $\separation=6$ in the sphere model. The hierarchy of IFMM is created with $\mu=40$. The meaning of the legends are the same as those in \autoref{tab:stat_sphereii10}.} %See \autoref{s:sphereii_sep6}.}
  \label{tab:stat_sep6}
  %
  \begin{tabular}{|c|HHr|r|r|rHH|}
    \toprule
    Level  & FMM & \multicolumn{5}{c}{nIFMM's groups} & &\\
    $\kappa$ & \#nodes & \#nodes & \#groups & Min & Ave & Max & $k=4$ & $k=32$\\
    \midrule
    2 & 56 & 56 & 56 & 1 & \prave{1.000000} & 1 & 144 & 1089\\
    3 & 272 & 272 & 112 & 2 & \prave{2.428571} & 3 & 100 & 529\\
    4 & 1160 & 1160 & 142 & 4 & \prave{8.169014} & 15 & 81 & 256\\
    5 & 4694 & 4742 & 181 & 5 & \prave{26.198895} & 52 & 64 & 144\\
    6 & 17640 & 18488 & 208 & 6 & \prave{88.884615} & 205 & 64 & 100\\
    7 & 58730 & 70896 & 216 & 8 & \prave{328.222222} & 802 & 64 & 81\\
    \bottomrule
  \end{tabular}\\[\baselineskip]
  % 
\end{table}

